Neural Models for Output-Space Invariance in Combinatorial Problems

Recently many neural models have been proposed to solve combinatorial puzzles by implicitly learning underlying constraints using their solved instances, such as sudoku or graph coloring (GCP). One drawback of the proposed architectures, which are often based on Graph Neural Networks (GNN), is that they cannot generalize across the size of the output space from which variables are assigned a value, for example, set of colors in a GCP, or board-size in sudoku. We call the output space for the variables as 'value-set'. While many works have demonstrated generalization of GNNs across graph size, there has been no study on how to design a GNN for achieving value-set invariance for problems that come from the same domain. For example, learning to solve 16 x 16 sudoku after being trained on only 9 x 9 sudokus. In this work, we propose novel methods to extend GNN based architectures to achieve value-set invariance. Specifically, our model builds on recently proposed Recurrent Relational Networks. Our first approach exploits the graph-size invariance of GNNs by converting a multi-class node classification problem into a binary node classification problem. Our second approach works directly with multiple classes by adding multiple nodes corresponding to the values in the value-set, and then connecting variable nodes to value nodes depending on the problem initialization. Our experimental evaluation on three different combinatorial problems demonstrates that both our models perform well on our novel problem, compared to a generic neural reasoner. Between two of our models, we observe an inherent trade-off: while the binarized model gives better performance when trained on smaller value-sets, multi-valued model is much more memory efficient, resulting in improved performance when trained on larger value-sets, where binarized model fails to train.

==> sections/abstract.tex <==
%We handle the problem of domain-size transfer in combinatorial optimization problems solved using neural models. 
Recent work has seen a surge in neural architectures for solving Constraint Satisfaction Problems (CSPs), such as Sudoku Puzzle. Most existing literature focuses on a fixed domain size of variables (\eg, number of digits in Sudoku), during training and testing. We are interested in the problem of domain-size invariance: Given the training and testing instances generated from a lifted CSP~\cite{joslin&roy97} for a fixed domain-size, can we learn models which generalize to solve instances generated from the same lifted CSP, but a different domain size? Here, only the structure of the problem (in terms of the constraint graph) is known, without the knowledge of the specific constraints.
%learn models which generalize to COP with unseen test sizes?
%train models which can solve the COP for unseen domain sizes?
%\ycom{It is not clear what is meant by problem size here. \eg, coloring a bigger 4 colorable graph at test time, after learning to color smaller graphs with 4 colors (graph size invariance) OR coloring a 5 colorable graph at test time? (domain size invariance). 
%Existing methods can achieve former but not later, and hence we should clarify this.}
%without even seeing a single example of the target size? 
%We emphasize this problem is different from transfer across varying size graphs in architectures such as GATs, where the set of values that a node can take remains constant during transfer. 
Our solution builds on Recurrent Relational Networks (RRNs) \cite{palm&al18}, which are non auto-regressive models, have
\ycom{that can be used}
been used for solving CSPs, and work by passing messages over the constraint graph representing. We enhance the RRNs in two different ways to solve the problem of domain-size invariance. Let $k$ and $k'$ denote the train and test \ycom{domain} sizes respectively. In our first approach, called the
{\em \binarymodel}, each variable in the CSP is replaced by $k$ different binary variables which are connected to each other in the constraint graph. Transfer happens naturally, since during inference, we need to create an $k'$-way representation with edge structure being the same as during training.
In our second approach, called the {\em \multimodel}, each value in the domain is explicitly represented by introducing a node in the graph, and are connected to each of the variable nodes. We pre-train $k'$ different embeddings, one for each value in test domain, by randomly sub-selecting an $k$ sized subset during each learning iteration. During inference, all the learned embeddings are used together. In both our architectures, we introduce different edge types for message passing, and an attention based mechanism, which are critical for good performance. Our experimental evaluation on 3 different CSPs demonstrates that both our models give respectable performance on 
%hitherto unaddressed 
the problem of domain-size transfer compared to generic neuro-symbolic models which fail to scale. Among two of our models, we observe an inherent trade-off: while the \binarymodel\ gives better performance when trained on smaller domain sizes, \multimodel\ is much more memory efficient, resulting in improved performance when trained on larger domain sizes, where \binarymodel\ fails to train. We present further insights into the performance of the two models.
%comparing the performance of the two models.
%into the relative performance of the two. % models.
%it results in better ping in improved performance when trained on larger domain sizes, . We present some insights in the possible reasons for the improved performance of binary model despite its simplicity.
%Both models give respectable performance on beats the multi-valued model by a huge marg

%binary model does better for smaller problem sizes, the two are comparable for larger test problems \ycom{This is true only if we ignore attention. With attention, binary model outperforms the best multi valued model by huge margins. }. 
%Further, multi-valued model is much more memory efficient due to its compact size, resulting in improved performance when trained on larger sizes, over which binary model can't be trained. 
%Both attention and edge typing are critical for the performance of both our models.

%Many neural architectures for solving combinatorial optimization problems have been proposed recently.
%They learn to solve Constraint Satisfaction Problems (CSPs) using the training data without explicit knowledge of constraints.
%In this work, our goal is to study `\textit{domain-size invariance}', in which the size of the domain from which variables are assigned a value differs during training and testing.
%The existing Graph Neural Network (GNN) based architectures can handle variance in the number of variables (graph-size invariance), but assume the domain into which variables are classified as fixed,
%\eg, while learning from $9 \times 9$ sudoku, RRN \cite{palm&al18} classify each of the $81$ sudoku cells into $9$ classes, and hence can't solve a $10 \times 10$ sudoku puzzle that would require classification over domain size $10$.
%Our contribution is two folds: first, we introduce the notion of \textit{`domain-size invariance'} for neural architectures trained to solve combinatorial optimization problems.
%Second, we propose two GNN based architectures to achieve domain-size invariance.
%The first architecture binarizes the problem by replacing each variable, that takes value from domain-size $k$, with $k$ new binary variables.
%This increases the original graph size by a factor of $k$, but makes the learning agnostic to the domain-size, thus exploiting the graph-size invariance of GNNs to achieve domain-size invariance.
%To address the increase in graph size, we propose our second architecture that introduces only $k$ new `\textit{value nodes}' in the graph.
%Message passing with shared parameters handles the different number of values nodes, thus achieving domain-size invariance.
%Experiments on three different tasks evaluate the effectiveness of the two methods.

==> sections/abstract_m.tex <==
Recent work has seen a surge in neural architectures for solving Constraint Satisfaction Problems (CSPs), such as Sudoku Puzzle, where the explicit constraints are not known, and instead learned from data. 
Most existing literature focuses on a fixed domain size of variables (\eg, number of digits in Sudoku), during training and testing. 
We extend this work by studying domain-size invariance in a Lifted CSP \cite{joslin&roy97}: given training data of ground CSPs from one domain-size, can we learn neural models that generalize to instances of the same lifted CSP but from a different domain size?
We propose two solutions for our problem on top of Recurrent Relational Networks (RRNs) \cite{palm&al18}, which model this problem in fixed domain-size setting. 
Our first solution converts each (multi-valued) CSP variable into multiple Boolean variables -– one for each value in the domain. 
Our \emph{binarized} problem is now naturally domain-size invariant, because it uses only two values, `0' and `1'. 
In our second solution, we operate directly on multi-valued problem, and represent each value in the domain as a separate node in the graph. We achieve domain size-invariance by training embeddings for a larger number of values than present in training problems.
In both solutions, we supplement RRN with additional components -- an attention module and a loss term. 
%that make substantial difference in final performance.   
Our experimental evaluation on three different lifted CSPs (Sudoku, Graph Coloring and Futoshiki) demonstrates that both our %models perform well on our novel problem, compared to generic neural reasoners, which fail to scale. We also compare the two 
models perform well on our novel problem, compared to a generic neural reasoner
%\todo{P:changed this line slightly to be specific that we compare with a single reasoner, and instead of fails to scale, perform significantly worse}, 
which performs significantly worse. We also compare the two models along axes of performance and scalability, and discuss their individual strengths and weaknesses.
%\todo{M: can we say more?}

%Between our two solutions, we observe an inherent trade-off: while our first solution gives better performance when trained on smaller domain sizes, our second solution is much more memory efficient, resulting in improved performance when trained on larger domain sizes. 
%We present further insights into the performance of the two models.

\begin{comment}
Recently many neural models have been proposed to implicitly learn constraints using solved instances of an underlying puzzle or a combinatorial problem, such as sudoku or graph coloring (GCP), and thereby learn to solve the problem.
One drawback of the proposed architectures, such as SATNet \cite{}, or Recurrent Graph Neural Network (GNN) \cite{other than RRN}, is that they can’t generalize across the size of the set from which values are assigned to the variables, for example, set of colors in a GCP, or board-size in sudoku. We call the set of values as ‘value-set’. While many works have demonstrated generalization of GNNs across graph size, there has been no study on how to design a GNN for achieving value-set invariance for problems that come from the same domain. For example, learning to solve 16 x 16 sudoku after being trained on only 9 x 9 sudokus, or coloring a 7 colorable graph after training on 4 colorable graphs.
In this work, we propose two extensions of a recently proposed GNN based architecture, RRN \cite{}, to achieve value-set invariance. 
Our first approach exploits the graph-size invariance of GNNs by converting a multi-class node classification problem into a binary node classification problem. 
Our second approach works directly with multiple classes by adding multiple nodes corresponding to the values in the value-set, and then connecting variable nodes to value nodes depending on the problem initialization.
In both solutions, we supplement RRN with additional components – an attention module and a loss term. Our experimental evaluation on three different combinatorial problems (Sudoku, Graph Coloring and Futoshiki) demonstrates that both our models perform well on our novel problem, compared to a generic neural reasoner which performs significantly worse. We also compare the two models along axes of performance and scalability, and discuss their individual strengths and weaknesses.

\end{comment}


==> sections/abstract_m_coopy.tex <==
Recent work has seen a surge in neural architectures for solving Constraint Satisfaction Problems (CSPs), such as Sudoku Puzzle, where the explicit constraints are not known, and instead learned from data. Most existing literature focuses on a fixed domain size of variables (\eg, number of digits in Sudoku), during training and testing. We extend this work by studying domain-size invariance in a Lifted CSP \cite{joslin&roy97}: given training data of ground CSPs from one domain-size, can we learn neural models that generalize to instances of the same lifted CSP but from a different domain size? We propose two solutions for our problem on top of Recurrent Relational Networks (RRNs) \cite{palm&al18}, which model this problem in fixed domain-size setting. Our first solution converts each (multi-valued) CSP variable into multiple Boolean variables -– one for each value in the domain. Our \emph{binarized} problem is now naturally domain-size invariant, because it uses only two values, `0' and `1'. In our second solution, we operate directly on multi-valued problem, and represent each value in the domain as a separate node in the graph. We achieve domain size-invariance by training embeddings for a larger number of values than present in training problems. In both solutions, we supplement RRN with additional components -- an attention module and a loss term. Our experimental evaluation on three different lifted CSPs (Sudoku, Graph Coloring and Futoshiki) demonstrates that both our models perform well on our novel problem, compared to a generic neural reasoner which performs significantly worse. We also compare the two models along axes of performance and scalability, and discuss their individual strengths and weaknesses.


==> sections/abstract_orig.tex <==
Many neural architectures for solving combinatorial optimization tasks have been proposed recently.
They can be thought of as learning to solve a particular kind of Constraint Satisfaction Problem (CSP) from many of its solved instances, without explicitly knowing the constraints, \eg, solving a $9 \times 9$ sudoku puzzle.
However, most of the recent architectures, \eg, SATNET \cite{wang&al19}, RRN \cite{palm&al18}, can not solve $k' \times k'$ sudoku puzzles if they are trained on $k \times k$ puzzles, with $k' \neq k$. 
\citet{palm&al18} cast it as $k = 9$ way multi-class classification for each sudoku cell, thereby fixing the `domain' from which variables of the CSP can take value.
In this work, we address this issue.
Our contribution is two folds.
First, we formally define the task of zero-shot neural learning for combinatorial problems such that at test times the variables have to be classified into domains of size larger than those observed during training.
We call it `\textit{domain-size invariance}'.
Second, we propose two Graph Neural Network (GNN) based architectures to achieve `\textit{domain size invariance}'.
In our first architecture, we construct a new bigger graph, $\bingraph$, with $kn$ nodes, from the original graph $\graph$ with $n$  nodes,  each to be classified into $k$ classes.
Instead of classifying each node in $\graph$ directly, we learn to classify each node in $\bingraph$ into $\{0,1\}$, making the learning task agnostic to domain size $k$.
At test time, with $k' \neq k$, only the graph size changes, which any standard GNN architecture can handle gracefully.
Note that the size of $\bingraph$ is at least $k$ times more than $\graph$, increasing the inference time as well as the GPU memory it takes,  which may become restrictive.
To address this, in our second architecture, we augment the original graph $\graph$ with only $k$ additional value nodes, one corresponding to each class.
Message passing learns the embedding of the original variable nodes and the value nodes.
In the end, variable nodes are classified by computing their bi-linear similarity with the value nodes.
Experiments on $3$ different tasks demonstrate the effectiveness of our two proposed methods for achieving domain-size invariance.


==> sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We have provided extensive experimental evidence for the claims made in the abstract and introduction. Refer to Section \ref{exps} for experimental results and discussion}
  \item Did you describe the limitations of your work?
    \answerYes{See discussion on Computational Complexity and Learning Challenges with the multi-valued model in Section \ref{Res-Dis}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{At the current stage, the work has a very limited scope of impacting society and thus the discussion is not relevant. }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{We do not present theoretical results in our work.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{We do not present theoretical results in our work.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We plan to make our data and code publicly available on acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Refer to the Section \ref{exps}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We have reported the standard deviation for all experiments over three runs by varying the random seed. Refer to \Cref{tab:futo:acc}, \Cref{tab:gcp:acc}, and \Cref{tab:sudoku:acc}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Refer to Section \ref{Exp and Baseline} for details on compute}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Citations have been provided for all relevant existing assets which were used in the work. For example, we cite \citet{palm&al18} and \cite{perron&furnon19} in Section \ref{tasks-datasets} for their dataset and library respectively}
  \item Did you mention the license of the assets?
    \answerNA{All assets that we have used are open-source and have been cited appropriately.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We plan to make our data and code publicly available on acceptance.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{None of the datasets used in the work contain any personal data. Existing datasets used are public in nature and have been cited appropriately.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{The datasets used have no personal data.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix


==> sections/discussion.tex <==
\ycom{
\section{Discussion}

\subsection{Size-Generalization of GNNs}

Our work relies heavily on the assumption that GNNs generalize across size. 
Here we briefly discuss the papers that question the same.
The existing set of papers (and results) in this line of research can be broadly divided into two sub-classes. The first set of results talk about the representation power of GNNs to handle various graph sizes. The second set of results talk about learnability issues with GNNs under varying train/test distributions. We look at some of the results below and try to explain why GNNs in our case are able to generalize well, both in terms of representation power, as well as learnability.

\textbf{Representation Power:} We hypothesize that there are two design choices that are helping us gain good representation power: 1. Ability to create a deep network without blowing up the number of parameters because of weight tying across layers, and 2. Preassigned class labels to some of the variables which act as node features and help in breaking the symmetry. We argue it on the basis of Theorem 4.2 in Yehudai et al. [ICML 2021], which proves that there exists a (d+3) layered GNN that can distinguish between nodes having different local structure (local structure is quantified via  d-patterns that can be thought of as a generalization of node degree to d-hop neighborhood). Hence, to be able to distinguish between nodes on the basis of a GNN, all we need to do is ensure that different nodes have different d-patterns. This can be achieved in 2 ways: 1. By increasing d, e.g. two nodes may have the same degree and hence the same  1-pattern, but their neighbors may have different degrees, which will lead to different 2-pattern for these two nodes. 2. By assigning node features, e.g. two nodes may have the same degree, but their neighbors may have different node features, leading to a different 1-pattern for them as d-pattern also takes initial node features into account. 
In addition, Tang et al. [Neurips 2020] also argue that one way of increasing the representation power of GNNs is by increasing their depth, and it achieves the same by proposing IterGNN that applies the same GNN layer for an adaptive number of iterations depending on the input graph. This is equivalent to tying the weights of different layers as in RRNs, as well as in our models. 

*Learnability:* With respect to learnability,  Yahudai et al. prove the existence of a ‘bad’ local minima that overfits on train data but fails on test samples that have unseen d-patterns. Our test dataset clearly has unseen d-patterns (e.g. nodes in 16 x 16 sudoku have different degrees than nodes in 9 x 9 sudoku), but our models still generalize. We note that Yehudai et al. only talks about the existence of some bad local minima, but does not rule out the possibility of the existence of other good local minima, which could generalize well, despite differences in local structure between train and test sets. This goes into the whole learnability argument, and whether we can find such not-so-bad local minimas (which presumably exist since the possibility has not been ruled out). One aspect that possibly comes to our rescue is that, unlike most GNN architectures, our design is recurrent in nature, i.e., parameters are tied across different GNN layers as inspired by Palm et al. [Neurips 2018]). Parameter tying assumption, possibly helps us in learnability, since the recurrence can be seen as a form of regularization, avoiding overfitting (or getting stuck in bad local minima). Exploring this further is a direction for future work.

In addition to Yehudai et al., Bevilacqua et al. [ICML 2021] deal with varying train/test distributions by proposing a size invariant representation of graphs. Their approach focuses on graph classification tasks, and is limited to creating size invariant representations for the entire graph. The theoretical claims presented in their paper primarily focus on the limitation of standard GNN based formulations for generalizing across sizes for graph classification tasks. On the other hand, we are interested in learning representations for each node in the graph for node classification, and it is not clear how the claims, as well as techniques proposed in the paper, extend to our setting. 


}

==> sections/results_discussion_before_p.tex <==
\subsection{Results and Discussion} 
\label{Res-Dis}
\begin{wrapfigure}{r}{0.3\linewidth}
\vspace{-3ex}
% \begin{figure}[h!]
  \centering
  \begin{subfigure}[b]{0.8\linewidth}
    \includegraphics[width=\linewidth]{figures/rtime-futo.png}
    \caption{Runtime}
  \end{subfigure} 
  \\
  \begin{subfigure}[b]{0.8\linewidth}
    \includegraphics[width=\linewidth]{figures/mem-used-futo.png}
    \caption{Memory}
  \end{subfigure} 
  \caption{Resource Utilization for Futoshiki} % across domains}
  \label{fig:resouce-util}
% \end{figure}
\vspace*{-1em}
\end{wrapfigure}
We report the accuracies over different sizes of value-set for 
Futoshiki, GCP and Sudoku in \Cref{tab:futo:acc}, \Cref{tab:gcp:acc}, and \Cref{tab:sudoku:acc}, respectively.
We first observe that NLM fails to train on Sudoku, and its performance is worse than one or both of our models for all experimental settings in Futoshiki and GCP. 
As expected, in Futoshiki, NLM model with depth $30$ fails to run on board sizes $11$ and $12$ and depth $15$ model fails to run on size $12$.
Note that both NLM and our \binarymodel\ work by binarizing the underlying puzzle, but we observe that \binarymodel\ shows significantly better generalization across size of value-set.
We note that NLM performs decently well for GCP even for the test graphs with chromatic number $k' = 7$. We attribute this to the fact that in our test data for $k'=7$, graphs are relatively small, with maximum 80 graph nodes, resulting in total $560$ binary objects in NLM, which is similar to the maximum $400$ binary objects that it trains over ($k$=4, max 100 nodes).

\textbf{Comparison between \binarymodel\ and \multimodel:}
Comparing our two models, we first observe that both the models achieve similar performance on the value-set over which they are trained. However,  \binarymodel\ obtains much better generalization than the \multimodel.
We also observe that the standard deviation of the \textit{board accuracy} increases significantly as the size of value-set increases, whereas the \textit{pointwise accuracy} is relatively stable. This is due to the high sensitivity of the board accuracy to pointwise accuracy: even if a single variable is incorrectly assigned in a puzzle, its contribution towards board accuracy goes to 0, whereas it still contributes positively towards pointwise accuracy.

\textbf{Learning challenge with the \multimodel:} 
We observe that the generalization ability of the \multimodel\ is worse than the \binarymodel. 
We hypothesise that it is 
%due to the fact that 
because
\multimodel\ never gets to see all the value embeddings together while training. Moreover, the different combinations of $k$ out of $k'$ embeddings increase exponentially with $(k' - k)$, making it further difficult to train. 
To validate this, we train a \multimodel\ with only $7$ learnable embeddings for Futoshiki and observe that the board accuracy on $7$ board-size increases to $97.82\%$ (at par with \binarymodel) from $90.18\%$
which is achieved 
when trained with $12$ embeddings. 
%Similarly, a $9\times 9$ trained Sudoku, when fine-tuned on a small $15\times 15$ dataset leads to a massive jump in board accuracy from 26\% to 99\% on the $16\times 16$ test set.
This 
indicates that the inability to train value embeddings effectively is one of the key issues for multi-valued model.

\textbf{Computational complexity:}
In \cref{fig:resouce-util}, for the two models, we compare the average inference time and the GPU memory occupied (computed using {\tt torch.cuda.max\_memory\_allocated}  function) by a batch of 32 Futoshiki puzzles over value-sets of varying sizes.
As expected, the \multimodel\ is much more efficient, both in terms of time and memory. We expect this to become crucial when we have to train using data from a larger CSP, as the computational graph for \binarymodel\ may not even fit in the available GPU memory. 
%\sout{For instance, \binarymodel\ can only run $12$ message passing steps on a $15\times 15$ Sudoku, even with a batch size of $1$, whereas \multimodel\ easily fits $6$ train problems in a batch with $32$ message passing steps. We leave the comparison of our models on much larger training problems for the future.}
To validate this, we further fine-tune our best  \multimodel and \binarymodel on $24 \times 24$ Sudoku puzzles and test on $25$ board size (see appendix for properties of this dataset).
As expected, while training we couldn't run any message passing step for \binarymodel and thus it achieves $0\%$ board accuracy.
On the other hand,  \multimodel\ being memory efficient, could easily fit $6$ puzzles in a train batch and achieves board and pointwise mean (stdev) percentage accuracies of $43.77 (14.42)$ and $98.59 (0.12)$ respectively on 25 board-size.
In addition, its performance on 16 board-size improves drastically to 90.39 (3.49) and 99.46 (0.15), further demonstrating that \emph{Representation power} of \multimodel\ is as good as \binarymodel, but the major challenge is that of learnability. 
%\vspace{-1ex}
\iffalse
To validate this, we assume access to a train dataset for domain size $15$ in sudoku and fine-tune our \binarymodel\ and \multimodel\ trained on $9 \times 9$ puzzles. 
We could run only $12$ message passing steps when fine-tuning the \binarymodel\ on $15$ board size as the computational graph for it goes out of memory beyond $12$ steps, even with batch size $1$.
On the other hand, we could easily fit batch size 6 for the \multimodel\ even with $32$ message passing steps.
The board accuracy for the \multimodel\ on $16 \times 16$ puzzles jumps to $99\%$ from $25.93\%$, matching the performance of the \binarymodel.
\ycom{Isn't this experiment, instead supporting our 1st hypothesis in "Learning challenge with multi valued model"? I am not sure if this experiment is now validating the significance of being resource efficient.}
\fi

==> sections/s1_introduction.tex <==
\section{Introduction}
\label{intro}
The capability of neural models to perform symbolic reasoning is often seen as a step towards the framework for unified AI, i.e., building  end-to-end trainable system for tasks, which need to combine low level perceptual reasoning with high level reasoning,\cite{system-A-system-B}.
Neural networks are increasingly becoming popular for solving symbolic tasks that require higher level reasoning, \eg, neural theorem proving \cite{rocktaschel&al15,evans&al18}, playing blocks world \cite{dong&al19}, or solving SAT \cite{circuitSAT, neuroSAT, PDP}. 
%i.e., \eg, solving a sudoku puzzle where the input is given in the form of an image ~\cite{wang&al19}. 
%These advances are often seen as a step towards achieving the goal of a unified framework for Artificial Intelligence~\cite{}.
%in a unified framework for Artificial Intelligence, which may need to combine low level perceptual task with high level reasoning, \eg, solving a sudoku puzzle where the input is given in the form of an image ~\cite{wang&al19}. 
%representation of a  sudoku puzzle \cite{wang&al19}, in which we first need to identify the digits (perceptual task) and then use high level reasoning to solve the symbolic sudoku.   
With the aim to further advance this capability,  we focus on solving lifted
%\ycom{what is structured CSP? Is the relationship b/w classes giving it the structure? Modulo that, is it different from regular CSPs?}
Constraint Satisfaction Problems (CSPs)
%Our work focuses on one such high level reasoning task -- learning to solve structured CSPs, 
%combinatorial optimization problems 
without explicit knowledge of the rules or the constraints, but only with the knowledge of the constraint graph. In such settings, the underlying constraints of the problem need to be implicitly learned from the given training data \eg, SATNET[], RRNs~\cite{palm&al18}.
%the One can think of such tasks as solving a Constraint Satisfaction Problem (CSP) where the constraints are not known and need to be learnt or inferred using the training data.
Most of the current state-of-the-art neural models make the assumption of a fixed domain size: the domain from which variables are assigned values is assumed to be constant during training and testing. This is a significant limitation since it may not always be possible to generate sufficient training data for different problem sizes (\cite{Sudoku-problem-generation-issue}).
This is also a desirable goal, since as humans, we often find it natural to generalize to problems of unseen sizes once, we know how to solve similar problems of a different size.\pcom{reference?}
%are trained for solving problems of a given size, while keeping the structure of the problem same.
%taking cue from human learning, where once we learn to solve problems of a certain size, we can easily generalize to solving problems 

In response, we tackle the following problem: Given the training \sout{and testing} instances generated from a lifted CSP~\cite{joslin&roy97} for a fixed domain-size \ycom{train and test are from different domain-size}, can we learn models which generalize to solve instances generated from the same lifted CSP, but a different domain size? We assume  only the structure of the problem (in terms of the constraint graph) is known, without the knowledge of the specific constraints. For instance, we may be interested in learning to solve Sudoku simply by looking at pairs of \sout{unsolved and corresponding solved puzzles} \ycom{puzzles and corresponding solutions} of a given size. And during testing, we are interested in solving puzzles of a different size.
%board sizesAs an example, one may be interested in learning to solve Sudoku puzzles, of a size different from those during training.
%%Given a fixed CSP structure, and training instances for some domain size, can we learn models which generalize to solve instances with the same CSP structure, but a %different domain size? The structure of the problem is specified in a language similar to finite first-order logic, and stays constant during training and testing. 
%For instance, when solving Sudoku, the rules of the game can be specified in the beginning, 
%\ycom{but we are assuming no access to the rules. This may confuse the reader. I think we need to be more clear about what information is represented by the given graph? Can't we use the term 'primal constraint graph' for the underlying structured CSP? Note that we are not given the first order logic formula as well.}
%and should work independent of the domain size of the problem. We note that the neural model is given access only to the 'constraint graph' \cite{}, and not the specific nature of the constraints. Though this problem can in principle be addressed using general purpose neuro-symbolic architectures (e.g., NLMs), they fail to scale as shown in our experiments.
%To the best of our knowledge, this problem of domain size transfer for structured CSPs has not been handled in the literature using neural architectures.
%\ycom{NLM, DeepProbLog? Are they not addressing similar problem? Especially NLM which specifically talks about rules in first order logic.}
We build our solution on top of RRNs~\cite{palm&al18} which have been effectively used for solving CSPs, albeit for problems with fixed domain size. RRNs are non auto-regressive models, which assume a graph structure to be given, and employ message passing over the underlying graph, to iteratively obtain an approximate solution. The structure of the graph is derived from the structure of the underlying CSP, such that, variables involved in a constraint with each other are connected to each other in the constraint graph. 
%As stated earlier, in the current form, they can not generalize over test instances of sizes different from training. 
We describe below two ways to enhance the RRN architecture to bring the idea of domain-size invariance. Let 
$k,k'$ denote the training and test domain sizes, respectively, in the following description. 

{\em \BinaryModel:} Each variable in the CSP is represented by $k$ different binary variable nodes that are connected to each other. Binary nodes corresponding to two different variables are connected to each other, if the corresponding variables share constraints. Invariance can be achieved naturally, since during inference, we need to create a $k'$-way representation with rest of the graph structure being the same as during training. Since all the variables in the resulting model are binary, we train an embedding for `0' and `1'. %We refer to this as \binarymodel\ for domain-size transfer, since the underlying variables are binarized for the task of transfer learning. 
Though this model is simplistic in nature, it suffers the problem of memory explosion: $O(nk^2)$ %\ycom{at least $O(nk^2)$} 
edges have to be introduced while constructing the underlying graph, $n$ being the number of variables in the original CSP. 
%for every variable in the original CSP. %$n$ being the number of variables in the original CSP. 
This can be a limiting factor when training on problems of large sizes. %In our second approach, referred to as 

\noindent {\em \MultiModel:} We introduce one {\em variable node} for every variable in CSP, which can take values from the underlying domain. Additionally, we introduce a node for every value in the domain of the problem, referred to as a {\em value node}. Each variable node is connected to every possible value node. Variable nodes corresponding to variables which appear in the same constraint are connected to each other. For the task of transfer, we learn as many embeddings, as there are values in the target (test) domain size. Since $k \neq k'$, and we are training over instances of size $k$, we circumvent this problem by randomly sub-selecting a $k$ sized subset during each learning iteration. This random sub-selection exploits the symmetry of domain values across instances.~\footnote{We address the issue separately when there may existing additional relations between values of the domain, making them symmetric only under certain conditions.} During inference, all the learned embeddings are used together. 

We introduce different edge types in the constraint graph based which lifted constraint an edge comes from. This helps in learning different messages for different functionalities. We also introduce an attention based mechanism to give different (learned) importance to different neighbors in the graph. Similar to RRNs, message passing is performed in a recurrent fashion to compute the final node embeddings, which are decoded into values.

We perform extensive experimental evaluation on there different structured CSPs: Graph Coloring (GP)~\cite{}, Futoshiki~\cite{}, and Sudoku~\cite{}. We compare two of our models with an NLM~\cite{} baseline which fails to scale for most test sizes used in our experiments.
%We note that there are no existing neural baselines which directly solve the problem of domain-size transfer.\vcom{Remove this in light of NLM?} 
While \binarymodel\ performs better when trained on lower domain sizes, presumably due to the simplicity of the underlying graph over which messages are passed, \multimodel\ is much more memory efficient, and can perform better when trained on larger problems, over which binary model fails to fit in memory. We also present additional insights and discussion into the (relative) performance of the two models.

%constrained structure of the problem
%to gradually reach the solution 
%As our first attempt to solve the above problem, we propose a {\em Binary model}, which binarizes each of the variable in the domain of the problem, into $k$ different binary variables, one for each value. 

%and hence such architectures fail to generalize over domain size. 
%For example, both RRN and SATNET models trained on $9 \times 9$ sudoku puzzles, can not solve $10 \times 10$ sudoku.
%RRN cast it as a node classification problem, where each of the 81 sudoku cells represented as nodes in the graph, are classified into 9 classes after many message passing steps. 
%Since the weights are shared, the architecture trained on $9 \times 9$ board, can run message passing on the bigger graph corresponding to $10 \times 10$ board. 
\begin{comment}

However, it fails to initialize the embedding of the nodes corresponding to sudoku cells filled with digit 10, as it learnt the embeddings for only 9 digits. 
Moreover, the final layer would still classify each node into 9 classes, and hence nodes corresponding to digit 10 will never be classified correctly.
On the other hand, SATNET represents sudoku as a learnable MAXSAT problem with a fixed number of Boolean variables, out of which some are  pre-assigned in the input and the rest are assigned a value by the network. Since the number of Boolean variables are fixed, it fails to run on a larger MAXSAT problem having more number of variables than present in the training samples.

In this work, we investigate two research questions: 
first, can we design neural architectures that achieve zero-shot domain-size in-variance while learning to solve a combinatorial optimization problem using training data consisting of solved problem instances in the smaller domain?
For example, coloring a $k'$ colorable graph after training only on $k$ colorable graphs with $k' > k$; solving $k' \times k'$ sudoku puzzles with $k' > k(=9) $, using training data consisting of only standard $9 \times 9$ puzzles.
Note that the rules or the constraints, if written in first order logic, would be identical across domain-size for all puzzles of a kind. However, the existing architectures fail to either represent or  classify an instance of the same puzzle from the larger domain.
In response, we design two GNN based architectures that are capable of solving problem instances from larger domain even when they are trained on similar problems from a fixed smaller domain.

Our first architecture, \binarymodel, exploits the observation that graph neural networks (GNNs) generalize very well across graph size. Similar to RRN, we cast it as a node classification problem, \ie, we run many message passing steps and in the end classify each node into one of the classes. But to exploit the invariance of GNNs on graph size for achieving domain-size invariance, we convert the multi-class classification into a binary node classification problem by creating a node, $\binnode{\jtr}{\ctr}$ for each (variable, class) pair $(\node^\jtr,\ctr)$, where $\jtr \in {1 \ldots n}$ and $\ctr \in {1 \ldots k}$ for a problem instance with $n$ variables and $k$  classes.
For example in $9 \times 9$ sudoku, each of the $n = 81$ cells represent a variable, and each variable is classified into $k = 9$ classes, resulting in a graph with total $729$ binary nodes.  
The binary nodes for a given class are connected by exactly the same edges as in the original graph formulation of the problem (as done in RRN). 
In additional to the problem specific edges, for each variable $\node^\jtr$, we connect all of its $k$ binary nodes, $\binnode{\jtr}{\ctr}, \ctr \in \{1 \ldots k\}$, with each other, resulting in a $k-$clique for each $\node^\jtr$. 
We distinguish these edges from the problem specific edges, resulting in a heterogeneous graph, unlike RRN. %Hence we use a different message function for each edge type.

One drawback of the \binarymodel\ is that for a $k$ class classification problem with $n$ variables and $|\edges|$ problem specific edges between them, it creates a graph with $kn$ nodes and $k|\edges| + nk(k-1)/2$ edges. 
This increases the graph size by a factor of $k$, resulting in increased inference time.
In our second architecture, \multiclassmodel, we try to overcome this issue by proposing a message passing neural network with only $n + k$ nodes and less than $|\edges| + nk$ edges.
For a problem with $n$ variables and $k$ classes, We introduce $k$ additional "value" nodes in the graph. A variable node which is pre-assigned in the input is connected to the corresponding class node and an un-assigned variable node is connected to all the class nodes. 
Now, how do we initialize the nodes such that we are able to solve problems over variable domain size?
Here, we first assume an upper limit, say $k_{max}$, on the size of the domain which we may encounter while testing. 
Accordingly, we learn $k_{max}$ different embeddings, instead of only $k$ that are required for puzzles in the train data.
To do so, we initialize the class nodes with any of the $k$ out of $k_{max}$ different embeddings. 
Pre-assigned variable nodes are initialized with the corresponding class embedding and empty variables nodes are initialized with the average of the selected $k$ embeddings.
Finally, each node is classified by computing its learnable bi-linear similarity with the corresponding class node.

As a second research question, we investigate 
if 
the proposed architectures can model any relationship that may exist between a pair of classes?
For example, in the board game of futoshiki, just like sudoku, we have to fill a $k \times k$ grid with numbers from $1 \ldots k$ such that a number does not repeat in the same row and column.
In addition, two grid cells, say $\node^\jtr$ and $\node^\ltr$, may have to satisfy $\relationfn(\pred[\jtr],\pred[\ltr])$, where $\pred[\jtr]$ and $\pred[\ltr]$ are the classes assigned to $\node^\jtr$ and $\node^\ltr$ respectively, and $R(\ctr_a,\ctr_b)$ is any binary function over classes, which evaluates to $1$ if $\relationfn$ holds for classes $\ctr_a$ and $\ctr_b$, \eg, $R(\ctr_a,\ctr_b) \equiv a < b$.
To formulate this, we need to model that $\relationfn(\ctr_a,\ctr_b) = 1$ iff $a < b$, where $\ctr_a$ and $\ctr_b$ are the classes representing the digits $a$ and $b$ respectively.

To model the relationship $\relationfn$ in the \binarymodel, for each variable $\node^\jtr$, we insert an edge, 
%of type 
$\binredge{}{}$,
between the binary nodes $\binnode{\jtr}{\ctr_a}$ and $\binnode{\jtr}{\ctr_b}$ corresponding to classes $\ctr_a$ and $\ctr_b$ whenever $\relationfn(\ctr_a,\ctr_b) = 1$. 

In \multiclassmodel, we use a separate graph neural network for generating the \textit{'relationship aware'} class embeddings.
It has  $k$ nodes corresponding to only the classes. 
Like \binarymodel, we insert edges,
$\redge{}{}$, between the class nodes $\ctr_a$ and $\ctr_b$ whenever $\relationfn(\ctr_a,\ctr_b) = 1$. 
As in the \multiclassmodel, the $k$ class nodes in this relationship aware embedding generator are initialized by randomly selecting any $k$ embeddings out of $k_{max}$.
The output of this embedding generator is used to initialize the class and variable nodes in the \multiclassmodel.

Below we enumerate the main contributions of our work:\\
1. We introduce domain-size in-variance as a desirable property for neural networks that solve combinatorial optimization problems. \\
2. We propose two simple yet effective GNN based architectures that can successfully solve  problem instances from larger domain size after training only on similar problem instances from a fixed smaller domain. \\
3. We present an effective way of modeling any binary relationship that may exist between the classes in the domain.\\
4. Finally, we compare the two proposed techniques through experiments on three combinatorial optimization tasks: Sudoku, Futoshiki and Graph Coloring Problem.
Since futoshiki has an additional constraint corresponding to 'less than' relationship, it allows us to also measure the effectiveness of our method to model the relationship between the classes in the domain.
\end{comment}

==> sections/s1_introduction_copy.tex <==
\section{Introduction}
\label{intro}
Neural networks are increasingly becoming popular for solving symbolic tasks that require higher level reasoning, \eg, neural theorem proving \cite{roch, evans&al18}, playing blocks world \cite{dong&al19}, solving SAT problems given in a particular form like CNF, DNF or circuits \cite{circuitSAT, neuroSAT, PDP}.
Neural architectures for such tasks may allow us to create an end-to-end trainable system in a unified  framework for Artificial Intelligence, which may need to combine low level perceptual task with high level reasoning, \eg, solving an image representation of a  sudoku puzzle \cite{wang&al19}, in which we first need to identify the digits (perceptual task) and then use high level reasoning to solve the symbolic sudoku.   
Our work focuses on one such high level reasoning task -- learning to solve combinatorial optimization problems without knowing the rules or the constraints. One can think of such tasks as solving a Constraint Satisfaction Problem (CSP) where the constraints are not known and need to be learnt or inferred using the training data.

Most of the current state-of-the-art neural models for solving combinatorial problems, \eg, SATNET \cite{wang&al19}, RRN \cite{palm&al18}, make a key assumption: the domain from which variables are assigned values is assumed to be the same during training and testing, and hence such architectures fail to generalize over domain size. 
For example, both RRN and SATNET models trained on $9 \times 9$ sudoku puzzles, can not solve $10 \times 10$ sudoku.
RRN cast it as a node classification problem, where each of the 81 sudoku cells represented as nodes in the graph, are classified into 9 classes after many message passing steps. 
Since the weights are shared, the architecture trained on $9 \times 9$ board, can run message passing on the bigger graph corresponding to $10 \times 10$ board. 
However, it fails to initialize the embedding of the nodes corresponding to sudoku cells filled with digit 10, as it learnt the embeddings for only 9 digits. 
Moreover, the final layer would still classify each node into 9 classes, and hence nodes corresponding to digit 10 will never be classified correctly.
On the other hand, SATNET represents sudoku as a learnable MAXSAT problem with a fixed number of Boolean variables, out of which some are  pre-assigned in the input and the rest are assigned a value by the network. Since the number of Boolean variables are fixed, it fails to run on a larger MAXSAT problem having more number of variables than present in the training samples.

In this work, we investigate two research questions: 
first, can we design neural architectures that achieve zero-shot domain-size in-variance while learning to solve a combinatorial optimization problem using training data consisting of solved problem instances in the smaller domain?
For example, coloring a $k'$ colorable graph after training only on $k$ colorable graphs with $k' > k$; solving $k' \times k'$ sudoku puzzles with $k' > k(=9) $, using training data consisting of only standard $9 \times 9$ puzzles.
Note that the rules or the constraints, if written in first order logic, would be identical across domain-size for all puzzles of a kind. However, the existing architectures fail to either represent or  classify an instance of the same puzzle from the larger domain.
In response, we design two GNN based architectures that are capable of solving problem instances from larger domain even when they are trained on similar problems from a fixed smaller domain.

Our first architecture, \binarymodel, exploits the observation that graph neural networks (GNNs) generalize very well across graph size. Similar to RRN, we cast it as a node classification problem, \ie, we run many message passing steps and in the end classify each node into one of the classes. But to exploit the invariance of GNNs on graph size for achieving domain-size invariance, we convert the multi-class classification into a binary node classification problem by creating a node, $\binnode{\jtr}{\ctr}$ for each (variable, class) pair $(\node^\jtr,\ctr)$, where $\jtr \in {1 \ldots n}$ and $\ctr \in {1 \ldots k}$ for a problem instance with $n$ variables and $k$  classes.
For example in $9 \times 9$ sudoku, each of the $n = 81$ cells represent a variable, and each variable is classified into $k = 9$ classes, resulting in a graph with total $729$ binary nodes.  
The binary nodes for a given class are connected by exactly the same edges as in the original graph formulation of the problem (as done in RRN). 
In additional to the problem specific edges, for each variable $\node^\jtr$, we connect all of its $k$ binary nodes, $\binnode{\jtr}{\ctr}, \ctr \in \{1 \ldots k\}$, with each other, resulting in a $k-$clique for each $\node^\jtr$. 
We distinguish these edges from the problem specific edges, resulting in a heterogeneous graph, unlike RRN. %Hence we use a different message function for each edge type.

One drawback of the \binarymodel\ is that for a $k$ class classification problem with $n$ variables and $|\edges|$ problem specific edges between them, it creates a graph with $kn$ nodes and $k|\edges| + nk(k-1)/2$ edges. 
This increases the graph size by a factor of $k$, resulting in increased inference time.
In our second architecture, \multiclassmodel, we try to overcome this issue by proposing a message passing neural network with only $n + k$ nodes and less than $|\edges| + nk$ edges.
For a problem with $n$ variables and $k$ classes, We introduce $k$ additional "value" nodes in the graph. A variable node which is pre-assigned in the input is connected to the corresponding class node and an un-assigned variable node is connected to all the class nodes. 
Now, how do we initialize the nodes such that we are able to solve problems over variable domain size?
Here, we first assume an upper limit, say $k_{max}$, on the size of the domain which we may encounter while testing. 
Accordingly, we learn $k_{max}$ different embeddings, instead of only $k$ that are required for puzzles in the train data.
To do so, we initialize the class nodes with any of the $k$ out of $k_{max}$ different embeddings. 
Pre-assigned variable nodes are initialized with the corresponding class embedding and empty variables nodes are initialized with the average of the selected $k$ embeddings.
Finally, each node is classified by computing its learnable bi-linear similarity with the corresponding class node.

As a second research question, we investigate 
if 
the proposed architectures can model any relationship that may exist between a pair of classes?
For example, in the board game of futoshiki, just like sudoku, we have to fill a $k \times k$ grid with numbers from $1 \ldots k$ such that a number does not repeat in the same row and column.
In addition, two grid cells, say $\node^\jtr$ and $\node^\ltr$, may have to satisfy $\relationfn(\pred[\jtr],\pred[\ltr])$, where $\pred[\jtr]$ and $\pred[\ltr]$ are the classes assigned to $\node^\jtr$ and $\node^\ltr$ respectively, and $R(\ctr_a,\ctr_b)$ is any binary function over classes, which evaluates to $1$ if $\relationfn$ holds for classes $\ctr_a$ and $\ctr_b$, \eg, $R(\ctr_a,\ctr_b) \equiv a < b$.
To formulate this, we need to model that $\relationfn(\ctr_a,\ctr_b) = 1$ iff $a < b$, where $\ctr_a$ and $\ctr_b$ are the classes representing the digits $a$ and $b$ respectively.

To model the relationship $\relationfn$ in the \binarymodel, for each variable $\node^\jtr$, we insert an edge, 
%of type 
$\binredge{}{}$,
between the binary nodes $\binnode{\jtr}{\ctr_a}$ and $\binnode{\jtr}{\ctr_b}$ corresponding to classes $\ctr_a$ and $\ctr_b$ whenever $\relationfn(\ctr_a,\ctr_b) = 1$. 

In \multiclassmodel, we use a separate graph neural network for generating the \textit{'relationship aware'} class embeddings.
It has  $k$ nodes corresponding to only the classes. 
Like \binarymodel, we insert edges,
$\redge{}{}$, between the class nodes $\ctr_a$ and $\ctr_b$ whenever $\relationfn(\ctr_a,\ctr_b) = 1$. 
As in the \multiclassmodel, the $k$ class nodes in this relationship aware embedding generator are initialized by randomly selecting any $k$ embeddings out of $k_{max}$.
The output of this embedding generator is used to initialize the class and variable nodes in the \multiclassmodel.

Below we enumerate the main contributions of our work:\\
1. We introduce domain-size in-variance as a desirable property for neural networks that solve combinatorial optimization problems. \\
2. We propose two simple yet effective GNN based architectures that can successfully solve  problem instances from larger domain size after training only on similar problem instances from a fixed smaller domain. \\
3. We present an effective way of modeling any binary relationship that may exist between the classes in the domain.\\
4. Finally, we compare the two proposed techniques through experiments on three combinatorial optimization tasks: Sudoku, Futoshiki and Graph Coloring Problem.
Since futoshiki has an additional constraint corresponding to 'less than' relationship, it allows us to also measure the effectiveness of our method to model the relationship between the classes in the domain.


==> sections/s3_methods_orig.tex <==
\section{Methods for Domain Size Invariance}

\textbf{Notation:
}
Let $\traindata = \{\queryi,\targeti\}_{\itr=1}^{m}$ be the $m$ training instances.
Each $\targeti$ has $n_\itr$ variables taking a value from a symbolic domain $\dspace_k$ of size $k$. 
Without loss of generality, one can assume $\dspace_k$ to be $\{1 \ldots k\}$.
Therefore,  $\targeti$ is an element from the structured combinatorial space $\tspace{k}{n_\itr}$ and can be thought of as a solution to an unknown Constraint Satisfaction Problem with some of the $n_\itr$ variables, say $g_\itr$, already grounded in the input $\queryi$. The remaining $n_\itr - g_\itr$ variables are masked as $0$ in the input $\queryi$ and thus
$\queryi \in \qspace{k}{n_\itr}$, where
$\dspace_k^{+}  = \dspace_k \cup \{0\}$.
%For example, for a $9 \times 9$ sudoku, $k = 9$, $n = 81$, $\dspace_k = \{1 \ldots 9\}$
We denote the $\jtr^{th}$ variable as $\queryi[\jtr]$ and its desired value as $\targeti[\jtr]$.

In addition to $\queryi$, we may also be given a primal constraint graph, $\graphi = (\verticesi,\edgesi)$, with the variables in $\queryi$ represented as vertices (nodes), and 
two variables, $\nodeij$ and $\nodeil$, are connected by an edge $\edgeijl$ if there is a constraint between them. 
For example, in the task of Graph Coloring Problem, $\graphi$ is nothing but the input graph and vary with each instance. 
On the other hand, for puzzles like Sudoku, the graph  remains the same across instances for a given board size with $n_\itr = k^2, \forall \itr$, and each variable (sudoku cell) is connected to all other variables in the same row, column, and grid \footnote{We may assume a fully connected graph in the lack of knowledge about the constraint graph. In such a case, the model will learn which edges are important and adjust its weights accordingly}.
%For puzzles like Futoshiki, the graph may contain edges of a special type repres


\textbf{Problem Definition:
} The task is to learn a neural model, $\model_\Theta$, with parameters $\Theta$, using the training data $\traindata$, such that, it is able to solve a query $\testquery \in \qspace{k'}{n'}$, with $k' > k$, given the corresponding primal constraint graph $\testgraph$.
Note that the variables in the test query $\testquery$
%not only has more number of variables than the queries in the training data, but also 
take values from a larger domain $\dspace_{k'}$ with size $k' > k$.

Next, we describe our two methods for achieving domain size invariance for solving combinatorial problems using message passing graph neural networks.

\subsection{Reformulation as Binary Classification: \binarymodel}

To achieve domain size invariance, in our first method we reformulate the task into a binary node classification problem.
We first describe how to construct a new graph, $\bingraph$, from a given primal constraint graph $\graph$.
Recurrent message passing is done on $\bingraph$.
Irrespective of the domain size $k$, each variable in the graph $\bingraph$ takes value from $\dspace_2 = \{0,1\}$, hence learning a model which is agnostic to the domain size for the variables in the training samples.
We then describe how to handle different relationships that may exist between the classes in the symbolic domain $\dspace_k$.
In the end, we briefly review the recurrent message passing graph neural network before moving on to our next method \multiclassmodel.

\subsubsection{Graph Construction for Message Passing}

Consider a query $\query \in \qspace{k}{n}$ with $n$ variables from $k$ sized domain $\dspace_k$, and its associated primal constraint graph $\graph = (\vertices, \edges)$.
%Corresponding to $\graph$, we first describe 
Construct a new graph, 
$\bingraph = (\binvertices, \binedges)$, with total $\lvert\binvertices\rvert = nk$ vertices and $|\binedges| = k|\edges| + nk(k-1)/2$ edges by following the steps below:



\begin{enumerate}
    \item For each of the $n$ nodes, $\nodej \in \vertices$, insert $k$  nodes, $\binnode{\jtr}{\ctr}, \ \forall \ctr \in \dspace_k$.

    \item For each edge $\edgejl \in \edges$ between nodes $\nodej$ and $\nodel$ in $\vertices$, insert $k$ edges, $\binedge{(\jtr,\ctr)}{(\ltr,\ctr)}, \ \forall \ctr \in \dspace_k$.
    
    \item For each $\jtr \in \{1 \ldots n\}$, add an edge $\binposnedge{(\jtr,\ctr_1)}{(\jtr,\ctr_2)}$ between nodes $\binnode{\jtr}{\ctr_1}$ and $\binnode{\jtr}{\ctr_2}$,
    $\forall \ctr_1, \ctr_2 \in \dspace_k$, and $\ctr_1 \neq \ctr_2$.
    
\end{enumerate}

In the original problem, each variable $\node^\jtr$ is classified into one of the $k$ classes in $\dspace_k$. 
In contrast, each variable $\binnode{\jtr}{\ctr}$, in the transformed problem, takes a value from $\dspace_2 = \{0,1\}$, making it agnostic to the domain size $k$.
For each of the $nk$ nodes $\binnode{\jtr}{\ctr}, \forall \jtr, \forall \ctr$ in $\bingraph$, the message passing network computes a probability, $Pr(\binnode{\jtr}{\ctr} ; \Theta)$, of classifying it as 1. 
The architecture for message passing network and computation of the probabilities is briefly discussed in \cref{subsec:msgpassing}.
To classify the original variables $\node^\jtr$ into one of the $k$ classes, we compare all the $k$ probabilities, $Pr(\binnode{\jtr}{\ctr} ; \Theta), \forall \ctr \in \dspace_k$, and assign to it the class corresponding to $\argmax_{\ctr \in \dspace_k} Pr(\binnode{\jtr}{\ctr} ; \Theta) $.

%Next, we briefly describe the message passing network to compute $Pr(\binnode{\jtr}{\ctr} ; \Theta)$ for each of the $nk$ nodes, $\binnode{\jtr}{\ctr}$, in the graph $\bingraph$.

\subsubsection{Handling Relationship Between Classes in \binarymodel}
Consider the board game of Futoshiki, in which a player has to fill in a $k \times k$ grid with numbers from $\dspace_k$ such that no number is repeated in a row and a column. 
In addition, there may exist a "$<$" constraint between two consecutive cells, implying that the number filled in the cell to the left of "$<$" has to be less than the number in the cell to its right. 
To satisfy this constraint, one needs to know all the pairs of classes between which "$<$" relationship holds.

In general, there may exist a binary function $\relationfn(\ctr_1, \ctr_1), \ctr_1, \ctr_2 \in \dspace_k$, such that it evaluates to $1$ whenever a relationship $\relation$ holds between classes $\ctr_1$ and $\ctr_2$.
In the input query $\query$, values assigned to any two variables $\query[\jtr]$ and $\query[\ltr]$ maybe constrained by relationship $\relation$, \ie, we wish to find a solution $\pred$ such that $\relationfn(\pred[\jtr], \pred[\ltr]) = 1$, where $\pred[\jtr]$ and $\pred[\ltr]$ are the values assigned to variables $\query[\jtr]$ and $\query[\ltr]$ respectively.
In the original problem, this can be represented by adding an edge $\redge{\jtr}{\ltr} \in \edges$ between the corresponding nodes $\nodej$ and $\nodel$ in $\graph$.

Now, to solve a puzzle with variables taking values from a larger domain size, one needs to model the relationship $\relation$ between all the classes, some of which might not have been seen during the training.
For this, we assume access to the complete binary relationship function $\relationfn$, along with the input query $\query$ and its corresponding primal constraint graph $\graph$. Note that $\graph$ also has relation edges $\redge{\nodej}{\nodel}$ between some of the pairs of nodes and the solution must satisfy the corresponding constraint.
To model this in \binarymodel, we augment the binary graph $\bingraph$ by the following edges:
\begin{enumerate}
  \setcounter{enumi}{3}
    \item For each relation edge $\redge{\jtr}{\ltr} \in \edges$ between nodes $\nodej$ and $\nodel$ in $\vertices$, insert $k$ edges, $\binredge{(\jtr,\ctr)}{(\ltr,\ctr)}, \ \forall \ctr \in \dspace_k$.
    
    \item For each $\jtr \in \{1 \ldots n\}$, add an edge $\binredge{(\jtr,\ctr_1)}{(\jtr,\ctr_2)}$ between nodes $\binnode{\jtr}{\ctr_1}$ and $\binnode{\jtr}{\ctr_2}$,
    $\forall \ctr_1, \ctr_2 \in \dspace_k $ such that  $
    \relationfn(\ctr_1,\ctr_2) = 1$.
\end{enumerate}

In all of our puzzles, we know that $k$ different nodes, $\binnode{\jtr}{\ctr} , \  \forall \ctr \in \dspace_k$ for a given variable $\node^\jtr$, represent different classes. 
We model this with a special relationship: $\alldiffrelation$, such that $\alldiffrelationfn(\ctr_1,\ctr_2) = 1$, whenever $\ctr_1  \neq \ctr_2, \forall \ctr_1, \ctr_2 \in \dspace_k$. 
Corresponding to $\alldiffrelation$, we insert the following edges:
\begin{enumerate}
  \setcounter{enumi}{5}
    \item For each $\jtr \in \{1 \ldots n \}$, add an edge $\bindiffedge{(\jtr,\ctr_1)}{(\jtr,\ctr_2)}$ between nodes $\binnode{\jtr}{\ctr_1}$ and $\binnode{\jtr}{\ctr_2}$,
    whenever $\ctr_1 \neq \ctr_2$, 
    $\forall \ctr_1, \ctr_2 \in \dspace_k$.
\end{enumerate}
    

\vcom{Mention that primal constraint graph is directed. 
Describe that the created graph is heterogenous: intra-diff vs inter-diff
Discuss about the drawbacks of the above methods: namely, huge size, impacting the inference time.
}

\subsubsection{Recurrent Message Passing for \binarymodel}
\label{subsec:msgpassing}
Once the graph $\bingraph$ is constructed, we run recurrent message passing for some predefined number of steps $T$. At each step, the hidden state of each node, $\binnode{\jtr}{\ctr}$, is updated by the messages received from its neighbors, and finally, based on its hidden state at step $T$, probability, $Pr(\binnode{\jtr}{\ctr} ; \Theta)$, of classifying it as 1 is computed.

\textbf{Initialization:
} 
The input features, $\inpfeature(\binnode{\jtr}{\ctr})$, for the nodes $\binnode{\jtr}{\ctr}, \forall \ctr$ are initialized based on the initial content of the variable $\query[\jtr], \forall \jtr$.  
If it is masked as 0, then $\inpfeature(\binnode{\jtr}{\ctr}) = -1, \forall \ctr \in \dspace_k$.
On the other hand, if $\query[\jtr]$ is preassigned a value $\hat{\ctr}$, then $\inpfeature(\binnode{\jtr}{\ctr}) = 0, \forall \ctr \neq \hat{\ctr}$, and $\inpfeature(\binnode{\jtr}{\hat{\ctr}}) = 1$.

\textbf{Edge Dependent Message Passing:}
The nodes communicate their current state via the messages sent to their neighbouring nodes across the edges.
The message depends not only on the current state of the sender and receiver, but also on the \textit{edge type} across which the message is sent. 
Specifically, for each of the edge types, $ \binedge{}{}$, $\binposnedge{}{}$, and $\binredge{}{}$, there is a separate message passing function,  $\msgfunction_{\binedge{}{}}$, 
$\msgfunction_{\binposnedge{}{}}$, and
$\msgfunction_{\binredge{}{}}$
respectively. We compute the message for each edge $\binedgetype{(\jtr,\ctr_1)}{(\ltr,\ctr_2)} \in \binedges$ as:

\begin{equation}
m_t \left(
    \binedgetype{(\jtr,\ctr_1)}{(\ltr,\ctr_2)} 
    \right) =  
    \msgfunction_{\binedgetype{}{}}
    \left(
    h_t \left( \binnode{\jtr}{\ctr_1} \right), 
    h_t \left( \binnode{\ltr}{\ctr_2} \right)
   \right), 
    \forall 
   \binedgetype{(\jtr,\ctr_1)}{(\ltr,\ctr_2)} \in \binedges, \ 
   \binedgetype{}{} \in \{\binedge{}{}, \binposnedge{}{}, \binredge{}{} \}  
\end{equation}

\textbf{Hidden State Update:}
Each node maintains its hidden state, $h_t(\binnode{\jtr}{\ctr})$, which is initialized by an embedding corresponding to its input feature. 
For each node, the incoming messages on the edges of the same type are aggregated by taking their weighted average. 
The weights, $a_t$, are computed using Bahdanau Attention \cite{} for $\binedge{}{}$ and $\binposnedge{}{}$, whereas messages across $\binredge{}{}$ are simply averaged:

\begin{equation}
    m_{t,\binedgetype{}{}}(\binnode{\jtr}{\ctr_1}) =
    \sum\limits_{\binedgetype{(\jtr,\ctr_1)}{(\jtr,\ctr_2)} \in \binedges} 
    a_t(\binedgetype{(\jtr,\ctr_1)}{(\jtr,\ctr_2)})
    m_t(\binedgetype{(\jtr,\ctr_1)}{(\jtr,\ctr_2)}) \ , \ \forall \binedgetype{}{} \in \{ \binedge{}{}, \binposnedge{}{}, \binredge{}{} \} 
\end{equation}

\vcom{Mention that attention is used only on a few edges?}

Finally, all messages, $m_{t,\binedgetype{}{}}(\binnode{\jtr}{\ctr}) \forall \binedgetype{}{} \in \{ \binedge{}{}, \binposnedge{}{}, \binredge{}{} \}$, are concatenated to create the input, $m_{t}(\binnode{\jtr}{\ctr})$ for each node, $\binnode{\jtr}{\ctr}$.
The hidden state at time step $t$ is updated by the following state update function to generate the state $h_{t+1}(\binnode{\jtr}{\ctr})$:
\begin{equation}
    h_{t+1}(\binnode{\jtr}{\ctr}) = 
    g\left(
    h_t(\binnode{\jtr}{\ctr}), m_{t}(\binnode{\jtr}{\ctr}),
    \inpfeature(\binnode{\jtr}{\ctr})
    \right), \forall \binnode{\jtr}{\ctr} \in \binvertices
\end{equation}

\textbf{Loss Computation, Target Values and Final Prediction: 
}
At each step $t$, we can compute the probability $Pr(\binnode{\jtr}{\ctr}; \Theta)$ of classifying a node $\binnode{\jtr}{\ctr}$ as $1$ by passing its hidden state through a scoring function $s$, \ie,
$Pr_t(\binnode{\jtr}{\ctr}; \Theta) = \sigma(s(h_t(\binnode{\jtr}{\ctr})))$, where $\sigma$ is the standard Sigmoid function.

The Binary Cross Entropy (BCE) loss for each node $\binnode{\jtr}{\ctr}$ is computed w.r.t. its target, $\bintarget[\jtr,\ctr]$, which is defined as $1$ whenever $\target[\jtr] = \ctr$ and $0$ otherwise.
Total loss at time step $t$ is nothing but the average BCE loss across all the nodes:

\begin{equation}
    \totalloss_t = \frac{1}{|\binvertices|}
    \sum\limits_{\binnode{\jtr}{\ctr} \in \binvertices}
    \left(
    \bintarget[\jtr,\ctr] \log\left(Pr_t(\binnode{\jtr}{\ctr}; \Theta)\right) + 
    \left(1 - \bintarget[\jtr,\ctr]\right)
    \log\left(1 - Pr_t(\binnode{\jtr}{\ctr}; \Theta)\right)
    \right)
\end{equation}

Like \citet{palm&al18}, while training we back-propagate through the loss at every time step $t \in \{1 \ldots T \}$ as it helps in learning a convergent message passing algorithm. 
Unlike them, during inference we run message passing till convergence upto a maximum number of steps $T'$.

Finally, for each original variable, $\node^\jtr$, we compare the $k$ probabilities for $\binnode{\jtr}{\ctr} \ \forall \ctr \in \dspace_k$, and assign to it the class corresponding to maximum probability, \ie, $\pred[\jtr] = \argmax_{\ctr \in \dspace_k} Pr_{T''}(\binnode{\jtr}{\ctr} ; \Theta) $, where $T'' \leq T'$ is the number of message passing steps till convergence. 


\subsubsection{Drawbacks of \binarymodel}

In the \binarymodel, notice that the constructed graph $\bingraph$ has $k|\vertices|$ nodes and at least $k|\edges| +  |\vertices|k(k-1)/2$ edges of type $\binedge{}{}$ and $\binposnedge{}{}$ respectively.
This increases the graph size by a factor of at least $k$. 
As a result, we may soon hit the memory limits of a GPU while training the \binarymodel\ with bigger problems. For example, the computation graph of a single $10 \times 10$ sudoku puzzle with $32$ message passing steps doesn't fit within $12$ GB memory of a K-40 GPU, making it impossible to train the model using sudoku puzzles of size greater than $10$. 
In addition, the bigger graph also results in increased inference time.
In the next model, we attempt to solve this bottleneck, though while training we need to make an assumption on the maximum domain size $k'$ of a test puzzle. 

\subsection{Augmenting the Multi-class Classification: \multiclassmodel }

To achieve domain size invariance in this method, we introduce $k$ new nodes of a different type in the original primal constraint graph $\graph$.
Each new node corresponds to a class in $\dspace_k$.
To distinguish them from the variable nodes, we call them \textit{value nodes}.
Notice that it makes the new graph heterogeneous not only w.r.t. edges, but also w.r.t. nodes, unlike the graph $\bingraph$ in \binarymodel.
After message passing, each variable node is classified by computing a bi-linear similarity score between its hidden state and the hidden state of each of the value nodes. 
It is assigned the class represented by the value node corresponding to the maximum similarity score. 

\subsubsection{Graph Construction for Message Passing:
}
Consider a query $\query \in \qspace{k}{n}$ with $n$ variables from $k$ sized domain $\dspace_k$, and its associated primal constraint graph $\graph = (\vertices, \edges)$.
Construct a new graph $\mcgraph  = (\mcvertices, \mcedges)$ with total $|\mcvertices| = n + k$ vertices and a maximum of $ |\edges| + nk$ edges by adding the following new nodes and edges in $\vertices$ and $\edges$ to get $\mcvertices$ and $\mcedges$ respectively:
\begin{enumerate}
    \item For each of the $k$ classes in $\dspace_k$, insert a \textit{value node}, 
    $\valuenode{\ctr}, \ \forall \ctr \in \dspace_k$.

    \item For each $\node^\jtr$, connect it with a value node $\valuenode{\ctr}$ if $\query[j] = \ctr$. 
    We denote such an edge as $\assignededge{\jtr}{\ctr}$.
    
    \item  If $\query[\jtr] = 0$, connect $\node^\jtr$ to all the value nodes $\valuenode{\ctr}, \ \forall \ctr \in \dspace_k$.
    We denote such edges as $\naedge{\jtr}{\ctr}$.
\end{enumerate}

Once the augmented graph $\mcgraph$ is constructed, we run recurrent message passing on it for $T$ steps and update the hidden state for both variable and value nodes.
At each step, we compute a score, $\bar{s}_t(\node^\jtr, \valuenode{\ctr})$, for assigning
value $\ctr$ to the node $\node^{\jtr}$. The scores are converted by a softmax layer into a probability simplex over $\dspace_k$.
Loss for each variable node $\node^\jtr$ at step $t$ is nothing but standard Cross Entropy loss of $Softmax(\bar{s}_t(\node^\jtr, \valuenode{\ctr})) \ \forall \ctr \in \dspace_k$ w.r.t. the target $\target[\jtr]$.


\subsubsection{Node Feature Initialization and Relationship Between Classes}

One important distinction between the message passing for \binarymodel\ and \multiclassmodel\ is the initialization of the node features.
Unlike \binarymodel, where each node is initialized with either 0, 1 or -1, 
%depending on the preassigned value of the corresponding variable in $\query$, 
here we wish to initialize each value node with a distinct feature.
But we can't learn only $k$ distinct features, because at test time, we may have $k' > k$ value nodes.
To circumvent this issue, we assume that we know $k_{max}$: the maximum domain size that we may expect during testing.
Accordingly, we intend to learn $k_{max}$ distinct feature embeddings.
To do so, we randomly select any $k$ of them for initializing the value nodes in a given training sample. 
Notice that for the different training samples in the same batch, or when the same training sample appears again in a different batch, a different random combination of $k$ features may get selected. 
Since each of the $k_{max}$ learnable feature embeddings get selected 
%with probability $1$ 
for one or the other sample while training, we end up learning all of them.


\textbf{Relationship between Classes:}
We wish to initialize the value node embeddings such that they are aware of any relationship $\relation$ that may exist between classes they represent.
To achieve this from any random selection of $k$ out of $k_{max}$ embeddings, we create a separate relationship graph, $\relationgraph = (\relationvertices, \relationedges)$, consisting of only the value nodes and relation edges.
Using the relationship function, $\relationfn(\ctr_1, \ctr_2)$, we construct it as follows: 
\begin{enumerate}
    \item For each class $\ctr \in \dspace_k$, create a node $\valuenode{\ctr}$
    \item Insert a relation edge, $\redge{\ctr_1}{\ctr_2}$ between $\valuenode{\ctr_1}$ and $\valuenode{\ctr_2}$ whenever $\relationfn(\ctr_1, \ctr_2) = 1$.
\end{enumerate}
Now each value node, $\valuenode{\ctr}$, represents a different class, which we model using relation $\alldiffrelation$ as in the \binarymodel, and insert the following edges in $\relationgraph$:
\begin{enumerate}
    \setcounter{enumi}{2}
    \item Insert an  edge, $\diffedge{\ctr_1}{\ctr_2}$ between $\valuenode{\ctr_1}$ and $\valuenode{\ctr_2}$ whenever $\ctr_1 \neq \ctr_2$.
\end{enumerate}

\textbf{Initialization:} Now even if the value nodes in $\relationgraph$ are initialized by any random choice of $k$ out of $k_{max}$ embeddings, we believe that first running message passing on $\relationgraph$ will eventually result in the embeddings that are `relationship-aware'.
Hence, we initialize the value nodes, $\valuenode{\ctr}$ in $\mcgraph$, using the `relationship-aware' embeddings of $\valuenode{\ctr}$ in $\relationgraph$.
The variable nodes that are preassigned a value in $\query$, are initialized by the embedding of the corresponding value node, \ie, if $\query[\jtr] = c$, then $\node^\jtr$ is initialized with the `relationship-aware' embedding of $\valuenode{\ctr}$.
On the other hand, the nodes corresponding to the masked variables are assigned the average of all `relationship-aware' embeddings.

\subsubsection{Recurrent Message Passing for \multiclassmodel}

\textbf{Input Features: } To achieve domain size invariance upto domain size $k_{max}$, we keep  $k_{max}$ learnable input features: $\mcinputfeature(\ctr) \  \forall \ctr \in \{1 \ldots k_{max} \}$. 

\textbf{Message Passing on $\relationgraph$ for generating `relationship-aware' embeddings:} 
For each query $\query$, select a $k-$permutation, $\perm_\query$, of $k_{max}$.
Initialize the hidden state, $\rghidden_0(\valuenode{\ctr})$, of $\valuenode{\ctr}$ in  $\relationgraph$  with $\mcinputfeature(\perm_\query[\ctr]), \ \forall \ctr \in \dspace_k$.
At step $t$, update the hidden state, $\rghidden_t(\valuenode{\ctr})$, of each of the value nodes in $\relationgraph$, by the average message, $m_t(\valuenode{\ctr})$, received across edges of type $\redge{}{}$: $\rghidden_{t+1}(\valuenode{\ctr}) = \rgupdatefn(\rghidden_t(\valuenode{\ctr}), m_t(\valuenode{\ctr}), \mcinputfeature(\perm_\query[\ctr]))$, 
where $\rgupdatefn$ is the hidden state update function. Like \cite{palm&al18}, it always take the initial hidden state as one of the inputs.
%where $\mcinputfeature(\perm_\query[\ctr]))$ is the initial node feature. 
Notice that the message, $m_t(\valuenode{\ctr})$, is the average of the messages, $\msgfunction_{\redge{}{}}(\rghidden_t(\ctr), \rghidden_t(\ctr_1)) \ \forall \redge{\ctr}{\ctr_1} \in \relationedges$, where $\msgfunction_{\redge{}{}}$ is the message passing function for edge type $\redge{}{}$.
The same function is used during the message passing in $\mcgraph$ for computing messages across edges of type $\redge{}{}$.
The hidden states are updated for $T_R$ steps and the final embeddings, $\rghidden_{T_R}(\valuenode{\ctr}) \ \forall \ctr \in \dspace_k$, are used as `relationship-aware' embeddings for initializing the hidden state of both variable nodes, $\node^\jtr$, and value nodes, $\valuenode{\ctr}$ in the graph $\mcgraph$.

\textbf{Initialization:} 
Initialize the hidden state, $h_0(\valuenode{\ctr})$, for each value node $\valuenode{\ctr}$ in $\mcgraph$, with $\rghidden_{T_R}(\ctr), \ \forall \ctr \in \dspace_k$.
For each variable node $\node^\jtr$, if $\query[\jtr] = \ctr$, then initialize its hidden state, $h_0(\node^\jtr)$, with $\rghidden_{T_R}(\ctr)$.
Otherwise, if $\query[\jtr] = 0$, then initialize $h_0(\node^\jtr)$ with $(1/k)\sum_{
\ctr \in \dspace_k} \rghidden_{T_R}(\ctr)$.

\textbf{Message Passing in $\mcgraph$:}
At time step $t$, similar to \binarymodel, each node receives messages from its neighbors, that are aggregated based on the edge type.
For each node, the aggregated messages, $m_{t,\edgetype{}{}}(\node^\jtr)$, for different edge types, $\edgetype{}{} \in \{\edge{}{}, \redge{}{},  \assignededge{}{}, \naedge{}{} \}$, are stacked to create, $m_t(\node^\jtr)$, which updates the hidden state as:
\begin{equation}
    h_{t+1}(\node^\jtr) = 
    g\left(
    h_t(\node^{\jtr}), m_{t}(\node^{\jtr}),
    h_0(\node^{\jtr})
    \right), \forall \node^{\jtr} \in \mcvertices
\end{equation}


\textbf{Loss Computation and Final Prediction:}
At time step $t$, a scoring function, $\bar{s}$, computes a score for assigning a value $\ctr$ to a variable $\node^\jtr$ based on the hidden state of corresponding value and variable nodes: $\bar{s}_t(\node^\jtr,\valuenode{\ctr}) = s(h_t(\node^\jtr), h_t(\valuenode{\ctr}))$.
For each variable node, a softmax converts these scores into probabilities over the classes $\ctr \in \dspace_k$, \ie, $Pr(\node^\jtr,\ctr) = Softmax(\bar{s}_t(\node^\jtr,\valuenode{\ctr})), \  \forall \ctr \in \dspace_k$.
Total loss at step $t$ is nothing but the average of standard Cross Entropy over variable nodes:
$L_t= - \frac{1}{|\vertices|}\sum_{\node^\jtr \in \vertices} \log(Pr(\node^\jtr, \target[\jtr]))$. 


==> sections/s3_methods_origv2.tex <==
\section{Methods for Domain Size Invariance}

\textbf{Notation:
}
Let $\traindata = \{\queryi,\targeti\}_{\itr=1}^{m}$ be the $m$ training instances.
Each $\targeti$ has $n_\itr$ variables taking a value from a symbolic domain $\dspace_k$ of size $k$. 
Without loss of generality, one can assume $\dspace_k$ to be $\{1 \ldots k\}$.
Therefore,  $\targeti$ is an element from the structured combinatorial space $\tspace{k}{n_\itr}$ and can be thought of as a solution to an unknown Constraint Satisfaction Problem with some of the $n_\itr$ variables, say $g_\itr$, already grounded in the input $\queryi$. The remaining $n_\itr - g_\itr$ variables are masked as $0$ in the input $\queryi$ and thus
$\queryi \in \qspace{k}{n_\itr}$, where
$\dspace_k^{+}  = \dspace_k \cup \{0\}$.
%For example, for a $9 \times 9$ sudoku, $k = 9$, $n = 81$, $\dspace_k = \{1 \ldots 9\}$
We denote the $\jtr^{th}$ variable as $\queryi[\jtr]$ and its desired value as $\targeti[\jtr]$.

In addition to $\queryi$, we may also be given a primal constraint graph, $\graphi = (\verticesi,\edgesi)$, with the variables in $\queryi$ represented as vertices (nodes), and 
two variables, $\nodeij$ and $\nodeil$, are connected by an edge $\edgeijl$ if there is a constraint between them. 
For example, in the task of Graph Coloring Problem, $\graphi$ is nothing but the input graph and vary with each instance. 
On the other hand, for puzzles like Sudoku, the graph  remains the same across instances for a given board size with $n_\itr = k^2, \forall \itr$, and each variable (sudoku cell) is connected to all other variables in the same row, column, and grid \footnote{We may assume a fully connected graph in the lack of knowledge about the constraint graph. In such a case, the model will learn which edges are important and adjust its weights accordingly}.
%For puzzles like Futoshiki, the graph may contain edges of a special type repres


\textbf{Problem Definition:
} The task is to learn a neural model, $\model_\Theta$, with parameters $\Theta$, using the training data $\traindata$, such that, it is able to solve a query $\testquery \in \qspace{k'}{n'}$, with $k' > k$, given the corresponding primal constraint graph $\testgraph$.
Note that the variables in the test query $\testquery$
%not only has more number of variables than the queries in the training data, but also 
take values from a larger domain $\dspace_{k'}$ with size $k' > k$.

Next, we describe our two methods for achieving domain size invariance for solving combinatorial problems using message passing graph neural networks.

\subsection{Reformulation as Binary Classification: \binarymodel}

To achieve domain size invariance, in our first method we reformulate the task into a binary node classification problem.
We first describe how to construct a new graph, $\bingraph$, from a given primal constraint graph $\graph$.
Recurrent message passing is done on $\bingraph$.
Irrespective of the domain size $k$, each variable in the graph $\bingraph$ takes value from $\dspace_2 = \{0,1\}$, hence learning a model which is agnostic to the domain size for the variables in the training samples.
We then describe how to handle different relationships that may exist between the classes in the symbolic domain $\dspace_k$.
In the end, we briefly review the recurrent message passing graph neural network before moving on to our next method \multiclassmodel.

\subsubsection{Graph Construction for Message Passing}

Consider a query $\query \in \qspace{k}{n}$ with $n$ variables from $k$ sized domain $\dspace_k$, and its associated primal constraint graph $\graph = (\vertices, \edges)$.
%Corresponding to $\graph$, we first describe 
Construct a new graph, 
$\bingraph = (\binvertices, \binedges)$, with total $\lvert\binvertices\rvert = nk$ vertices and $|\binedges| = k|\edges| + nk(k-1)/2$ edges by following the steps below:



\begin{enumerate}
    \item For each of the $n$ nodes, $\nodej \in \vertices$, insert $k$  nodes, $\binnode{\jtr}{\ctr}, \ \forall \ctr \in \dspace_k$.

    \item For each edge $\edgejl \in \edges$ between nodes $\nodej$ and $\nodel$ in $\vertices$, insert $k$ edges, $\binedge{(\jtr,\ctr)}{(\ltr,\ctr)}, \ \forall \ctr \in \dspace_k$.
    
    \item For each $\jtr \in \{1 \ldots n\}$, add an edge $\binposnedge{(\jtr,\ctr_1)}{(\jtr,\ctr_2)}$ between nodes $\binnode{\jtr}{\ctr_1}$ and $\binnode{\jtr}{\ctr_2}$,
    $\forall \ctr_1, \ctr_2 \in \dspace_k$, and $\ctr_1 \neq \ctr_2$.
    
\end{enumerate}

In the original problem, each variable $\node^\jtr$ is classified into one of the $k$ classes in $\dspace_k$. 
In contrast, each variable $\binnode{\jtr}{\ctr}$, in the transformed problem, takes a value from $\dspace_2 = \{0,1\}$, making it agnostic to the domain size $k$.
For each of the $nk$ nodes $\binnode{\jtr}{\ctr}, \forall \jtr, \forall \ctr$ in $\bingraph$, the message passing network computes a probability, $Pr(\binnode{\jtr}{\ctr} ; \Theta)$, of classifying it as 1. 
The architecture for message passing network and computation of the probabilities is briefly discussed in \cref{subsec:msgpassing}.
To classify the original variables $\node^\jtr$ into one of the $k$ classes, we compare all the $k$ probabilities, $Pr(\binnode{\jtr}{\ctr} ; \Theta), \forall \ctr \in \dspace_k$, and assign to it the class corresponding to $\argmax_{\ctr \in \dspace_k} Pr(\binnode{\jtr}{\ctr} ; \Theta) $.

%Next, we briefly describe the message passing network to compute $Pr(\binnode{\jtr}{\ctr} ; \Theta)$ for each of the $nk$ nodes, $\binnode{\jtr}{\ctr}$, in the graph $\bingraph$.

\subsubsection{Handling Relationship Between Classes in \binarymodel}
Consider the board game of Futoshiki, in which a player has to fill in a $k \times k$ grid with numbers from $\dspace_k$ such that no number is repeated in a row and a column. 
In addition, there may exist a "$<$" constraint between two consecutive cells, implying that the number filled in the cell to the left of "$<$" has to be less than the number in the cell to its right. 
To satisfy this constraint, one needs to know all the pairs of classes between which "$<$" relationship holds.

In general, there may exist a binary function $\relationfn(\ctr_1, \ctr_1), \ctr_1, \ctr_2 \in \dspace_k$, such that it evaluates to $1$ whenever a relationship $\relation$ holds between classes $\ctr_1$ and $\ctr_2$.
In the input query $\query$, values assigned to any two variables $\query[\jtr]$ and $\query[\ltr]$ maybe constrained by relationship $\relation$, \ie, we wish to find a solution $\pred$ such that $\relationfn(\pred[\jtr], \pred[\ltr]) = 1$, where $\pred[\jtr]$ and $\pred[\ltr]$ are the values assigned to variables $\query[\jtr]$ and $\query[\ltr]$ respectively.
In the original problem, this can be represented by adding an edge $\redge{\jtr}{\ltr} \in \edges$ between the corresponding nodes $\nodej$ and $\nodel$ in $\graph$.

Now, to solve a puzzle with variables taking values from a larger domain size, one needs to model the relationship $\relation$ between all the classes, some of which might not have been seen during the training.
For this, we assume access to the complete binary relationship function $\relationfn$, along with the input query $\query$ and its corresponding primal constraint graph $\graph$. Note that $\graph$ also has relation edges $\redge{\nodej}{\nodel}$ between some of the pairs of nodes and the solution must satisfy the corresponding constraint.
To model this in \binarymodel, we augment the binary graph $\bingraph$ by the following edges:
\begin{enumerate}
  \setcounter{enumi}{3}
    \item For each relation edge $\redge{\jtr}{\ltr} \in \edges$ between nodes $\nodej$ and $\nodel$ in $\vertices$, insert $k$ edges, $\binredge{(\jtr,\ctr)}{(\ltr,\ctr)}, \ \forall \ctr \in \dspace_k$.
    
    \item For each $\jtr \in \{1 \ldots n\}$, add an edge $\binredge{(\jtr,\ctr_1)}{(\jtr,\ctr_2)}$ between nodes $\binnode{\jtr}{\ctr_1}$ and $\binnode{\jtr}{\ctr_2}$,
    $\forall \ctr_1, \ctr_2 \in \dspace_k $ such that  $
    \relationfn(\ctr_1,\ctr_2) = 1$.
\end{enumerate}

In all of our puzzles, we know that $k$ different nodes, $\binnode{\jtr}{\ctr} , \  \forall \ctr \in \dspace_k$ for a given variable $\node^\jtr$, represent different classes. 
We model this with a special relationship: $\alldiffrelation$, such that $\alldiffrelationfn(\ctr_1,\ctr_2) = 1$, whenever $\ctr_1  \neq \ctr_2, \forall \ctr_1, \ctr_2 \in \dspace_k$. 
Corresponding to $\alldiffrelation$, we insert the following edges:
\begin{enumerate}
  \setcounter{enumi}{5}
    \item For each $\jtr \in \{1 \ldots n \}$, add an edge $\bindiffedge{(\jtr,\ctr_1)}{(\jtr,\ctr_2)}$ between nodes $\binnode{\jtr}{\ctr_1}$ and $\binnode{\jtr}{\ctr_2}$,
    whenever $\ctr_1 \neq \ctr_2$, 
    $\forall \ctr_1, \ctr_2 \in \dspace_k$.
\end{enumerate}
    

\vcom{Mention that primal constraint graph is directed. 
Describe that the created graph is heterogenous: intra-diff vs inter-diff
Discuss about the drawbacks of the above methods: namely, huge size, impacting the inference time.
}

\subsubsection{Recurrent Message Passing for \binarymodel}
\label{subsec:msgpassing}
Once the graph $\bingraph$ is constructed, we run recurrent message passing for some predefined number of steps $T$. At each step, the hidden state of each node, $\binnode{\jtr}{\ctr}$, is updated by the messages received from its neighbors, and finally, based on its hidden state at step $T$, probability, $Pr(\binnode{\jtr}{\ctr} ; \Theta)$, of classifying it as 1 is computed.

\textbf{Initialization:
} 
The input features, $\inpfeature(\binnode{\jtr}{\ctr})$, for the nodes $\binnode{\jtr}{\ctr}, \forall \ctr$ are initialized based on the initial content of the variable $\query[\jtr], \forall \jtr$.  
If it is masked as 0, then $\inpfeature(\binnode{\jtr}{\ctr}) = -1, \forall \ctr \in \dspace_k$.
On the other hand, if $\query[\jtr]$ is preassigned a value $\hat{\ctr}$, then $\inpfeature(\binnode{\jtr}{\ctr}) = 0, \forall \ctr \neq \hat{\ctr}$, and $\inpfeature(\binnode{\jtr}{\hat{\ctr}}) = 1$.

\textbf{Edge Dependent Message Passing:}
The nodes communicate their current state via the messages sent to their neighbouring nodes across the edges.
The message depends not only on the current state of the sender and receiver, but also on the \textit{edge type} across which the message is sent. 
Specifically, for each of the edge types, $ \binedge{}{}$, $\binposnedge{}{}$, and $\binredge{}{}$, there is a separate message passing function,  $\msgfunction_{\binedge{}{}}$, 
$\msgfunction_{\binposnedge{}{}}$, and
$\msgfunction_{\binredge{}{}}$
respectively. We compute the message for each edge $\binedgetype{(\jtr,\ctr_1)}{(\ltr,\ctr_2)} \in \binedges$ as:

\begin{equation}
m_t \left(
    \binedgetype{(\jtr,\ctr_1)}{(\ltr,\ctr_2)} 
    \right) =  
    \msgfunction_{\binedgetype{}{}}
    \left(
    h_t \left( \binnode{\jtr}{\ctr_1} \right), 
    h_t \left( \binnode{\ltr}{\ctr_2} \right)
   \right), 
    \forall 
   \binedgetype{(\jtr,\ctr_1)}{(\ltr,\ctr_2)} \in \binedges, \ 
   \binedgetype{}{} \in \{\binedge{}{}, \binposnedge{}{}, \binredge{}{} \}  
\end{equation}

\textbf{Hidden State Update:}
Each node maintains its hidden state, $h_t(\binnode{\jtr}{\ctr})$, which is initialized by an embedding corresponding to its input feature. 
For each node, the incoming messages on the edges of the same type are aggregated by taking their weighted average. 
The weights, $a_t$, are computed using Bahdanau Attention \cite{} for $\binedge{}{}$ and $\binposnedge{}{}$, whereas messages across $\binredge{}{}$ are simply averaged:

\begin{equation}
    m_{t,\binedgetype{}{}}(\binnode{\jtr}{\ctr_1}) =
    \sum\limits_{\binedgetype{(\jtr,\ctr_1)}{(\jtr,\ctr_2)} \in \binedges} 
    a_t(\binedgetype{(\jtr,\ctr_1)}{(\jtr,\ctr_2)})
    m_t(\binedgetype{(\jtr,\ctr_1)}{(\jtr,\ctr_2)}) \ , \ \forall \binedgetype{}{} \in \{ \binedge{}{}, \binposnedge{}{}, \binredge{}{} \} 
\end{equation}

\vcom{Mention that attention is used only on a few edges?}

Finally, all messages, $m_{t,\binedgetype{}{}}(\binnode{\jtr}{\ctr}) \forall \binedgetype{}{} \in \{ \binedge{}{}, \binposnedge{}{}, \binredge{}{} \}$, are concatenated to create the input, $m_{t}(\binnode{\jtr}{\ctr})$ for each node, $\binnode{\jtr}{\ctr}$.
The hidden state at time step $t$ is updated by the following state update function to generate the state $h_{t+1}(\binnode{\jtr}{\ctr})$:
\begin{equation}
    h_{t+1}(\binnode{\jtr}{\ctr}) = 
    g\left(
    h_t(\binnode{\jtr}{\ctr}), m_{t}(\binnode{\jtr}{\ctr}),
    \inpfeature(\binnode{\jtr}{\ctr})
    \right), \forall \binnode{\jtr}{\ctr} \in \binvertices
\end{equation}

\textbf{Loss Computation, Target Values and Final Prediction: 
}
At each step $t$, we can compute the probability $Pr(\binnode{\jtr}{\ctr}; \Theta)$ of classifying a node $\binnode{\jtr}{\ctr}$ as $1$ by passing its hidden state through a scoring function $s$, \ie,
$Pr_t(\binnode{\jtr}{\ctr}; \Theta) = \sigma(s(h_t(\binnode{\jtr}{\ctr})))$, where $\sigma$ is the standard Sigmoid function.

The Binary Cross Entropy (BCE) loss for each node $\binnode{\jtr}{\ctr}$ is computed w.r.t. its target, $\bintarget[\jtr,\ctr]$, which is defined as $1$ whenever $\target[\jtr] = \ctr$ and $0$ otherwise.
Total loss at time step $t$ is nothing but the average BCE loss across all the nodes:

\begin{equation}
    \totalloss_t = \frac{1}{|\binvertices|}
    \sum\limits_{\binnode{\jtr}{\ctr} \in \binvertices}
    \left(
    \bintarget[\jtr,\ctr] \log\left(Pr_t(\binnode{\jtr}{\ctr}; \Theta)\right) + 
    \left(1 - \bintarget[\jtr,\ctr]\right)
    \log\left(1 - Pr_t(\binnode{\jtr}{\ctr}; \Theta)\right)
    \right)
\end{equation}

Like \citet{palm&al18}, while training we back-propagate through the loss at every time step $t \in \{1 \ldots T \}$ as it helps in learning a convergent message passing algorithm. 
Unlike them, during inference we run message passing till convergence upto a maximum number of steps $T'$.

Finally, for each original variable, $\node^\jtr$, we compare the $k$ probabilities for $\binnode{\jtr}{\ctr} \ \forall \ctr \in \dspace_k$, and assign to it the class corresponding to maximum probability, \ie, $\pred[\jtr] = \argmax_{\ctr \in \dspace_k} Pr_{T''}(\binnode{\jtr}{\ctr} ; \Theta) $, where $T'' \leq T'$ is the number of message passing steps till convergence. 


\subsubsection{Drawbacks of \binarymodel}

In the \binarymodel, notice that the constructed graph $\bingraph$ has $k|\vertices|$ nodes and at least $k|\edges| +  |\vertices|k(k-1)/2$ edges of type $\binedge{}{}$ and $\binposnedge{}{}$ respectively.
This increases the graph size by a factor of at least $k$. 
As a result, we may soon hit the memory limits of a GPU while training the \binarymodel\ with bigger problems. For example, the computation graph of a single $10 \times 10$ sudoku puzzle with $32$ message passing steps doesn't fit within $12$ GB memory of a K-40 GPU, making it impossible to train the model using sudoku puzzles of size greater than $10$. 
In addition, the bigger graph also results in increased inference time.
In the next model, we attempt to solve this bottleneck, though while training we need to make an assumption on the maximum domain size $k'$ of a test puzzle. 

\subsection{Augmenting the Multi-class Classification: \multiclassmodel }

To achieve domain size invariance in this method, we introduce $k$ new nodes of a different type in the original primal constraint graph $\graph$.
Each new node corresponds to a class in $\dspace_k$.
To distinguish them from the variable nodes, we call them \textit{value nodes}.
Notice that it makes the new graph heterogeneous not only w.r.t. edges, but also w.r.t. nodes, unlike the graph $\bingraph$ in \binarymodel.
After message passing, each variable node is classified by computing a bi-linear similarity score between its hidden state and the hidden state of each of the value nodes. 
It is assigned the class represented by the value node corresponding to the maximum similarity score. 

\subsubsection{Graph Construction for Message Passing:
}
Consider a query $\query \in \qspace{k}{n}$ with $n$ variables from $k$ sized domain $\dspace_k$, and its associated primal constraint graph $\graph = (\vertices, \edges)$.
Construct a new graph $\mcgraph  = (\mcvertices, \mcedges)$ with total $|\mcvertices| = n + k$ vertices and a maximum of $ |\edges| + nk$ edges by adding the following new nodes and edges in $\vertices$ and $\edges$ to get $\mcvertices$ and $\mcedges$ respectively:
\begin{enumerate}
    \item For each of the $k$ classes in $\dspace_k$, insert a \textit{value node}, 
    $\valuenode{\ctr}, \ \forall \ctr \in \dspace_k$.

    \item For each $\node^\jtr$, connect it with a value node $\valuenode{\ctr}$ if $\query[j] = \ctr$. 
    We denote such an edge as $\assignededge{\jtr}{\ctr}$.
    
    \item  If $\query[\jtr] = 0$, connect $\node^\jtr$ to all the value nodes $\valuenode{\ctr}, \ \forall \ctr \in \dspace_k$.
    We denote such edges as $\naedge{\jtr}{\ctr}$.
\end{enumerate}

Once the augmented graph $\mcgraph$ is constructed, we run recurrent message passing on it for $T$ steps and update the hidden state for both variable and value nodes.
At each step, we compute a score, $\bar{s}_t(\node^\jtr, \valuenode{\ctr})$, for assigning
value $\ctr$ to the node $\node^{\jtr}$. The scores are converted by a softmax layer into a probability simplex over $\dspace_k$.
Loss for each variable node $\node^\jtr$ at step $t$ is nothing but standard Cross Entropy loss of $Softmax(\bar{s}_t(\node^\jtr, \valuenode{\ctr})) \ \forall \ctr \in \dspace_k$ w.r.t. the target $\target[\jtr]$.


\subsubsection{Node Feature Initialization and Relationship Between Classes}

One important distinction between the message passing for \binarymodel\ and \multiclassmodel\ is the initialization of the node features.
Unlike \binarymodel, where each node is initialized with either 0, 1 or -1, 
%depending on the preassigned value of the corresponding variable in $\query$, 
here we wish to initialize each value node with a distinct feature.
But we can't learn only $k$ distinct features, because at test time, we may have $k' > k$ value nodes.
To circumvent this issue, we assume that we know $k_{max}$: the maximum domain size that we may expect during testing.
Accordingly, we intend to learn $k_{max}$ distinct feature embeddings.
To do so, we randomly select any $k$ of them for initializing the value nodes in a given training sample. 
Notice that for the different training samples in the same batch, or when the same training sample appears again in a different batch, a different random combination of $k$ features may get selected. 
Since each of the $k_{max}$ learnable feature embeddings get selected 
%with probability $1$ 
for one or the other sample while training, we end up learning all of them.


\textbf{Relationship between Classes:}
We wish to initialize the value node embeddings such that they are aware of any relationship $\relation$ that may exist between classes they represent.
To achieve this from any random selection of $k$ out of $k_{max}$ embeddings, we create a separate relationship graph, $\relationgraph = (\relationvertices, \relationedges)$, consisting of only the value nodes and relation edges.
Using the relationship function, $\relationfn(\ctr_1, \ctr_2)$, we construct it as follows: 
\begin{enumerate}
    \item For each class $\ctr \in \dspace_k$, create a node $\valuenode{\ctr}$
    \item Insert a relation edge, $\redge{\ctr_1}{\ctr_2}$ between $\valuenode{\ctr_1}$ and $\valuenode{\ctr_2}$ whenever $\relationfn(\ctr_1, \ctr_2) = 1$.
\end{enumerate}
Now each value node, $\valuenode{\ctr}$, represents a different class, which we model using relation $\alldiffrelation$ as in the \binarymodel, and insert the following edges in $\relationgraph$:
\begin{enumerate}
    \setcounter{enumi}{2}
    \item Insert an  edge, $\diffedge{\ctr_1}{\ctr_2}$ between $\valuenode{\ctr_1}$ and $\valuenode{\ctr_2}$ whenever $\ctr_1 \neq \ctr_2$.
\end{enumerate}

\textbf{Initialization:} Now even if the value nodes in $\relationgraph$ are initialized by any random choice of $k$ out of $k_{max}$ embeddings, we believe that first running message passing on $\relationgraph$ will eventually result in the embeddings that are `relationship-aware'.
Hence, we initialize the value nodes, $\valuenode{\ctr}$ in $\mcgraph$, using the `relationship-aware' embeddings of $\valuenode{\ctr}$ in $\relationgraph$.
The variable nodes that are preassigned a value in $\query$, are initialized by the embedding of the corresponding value node, \ie, if $\query[\jtr] = c$, then $\node^\jtr$ is initialized with the `relationship-aware' embedding of $\valuenode{\ctr}$.
On the other hand, the nodes corresponding to the masked variables are assigned the average of all `relationship-aware' embeddings.

\subsubsection{Recurrent Message Passing for \multiclassmodel}

\textbf{Input Features: } To achieve domain size invariance upto domain size $k_{max}$, we keep  $k_{max}$ learnable input features: $\mcinputfeature(\ctr) \  \forall \ctr \in \{1 \ldots k_{max} \}$. 

\textbf{Message Passing on $\relationgraph$ for generating `relationship-aware' embeddings:} 
For each query $\query$, select a $k-$permutation, $\perm_\query$, of $k_{max}$.
Initialize the hidden state, $\rghidden_0(\valuenode{\ctr})$, of $\valuenode{\ctr}$ in  $\relationgraph$  with $\mcinputfeature(\perm_\query[\ctr]), \ \forall \ctr \in \dspace_k$.
At step $t$, update the hidden state, $\rghidden_t(\valuenode{\ctr})$, of each of the value nodes in $\relationgraph$, by the average message, $m_t(\valuenode{\ctr})$, received across edges of type $\redge{}{}$: $\rghidden_{t+1}(\valuenode{\ctr}) = \rgupdatefn(\rghidden_t(\valuenode{\ctr}), m_t(\valuenode{\ctr}), \mcinputfeature(\perm_\query[\ctr]))$, 
where $\rgupdatefn$ is the hidden state update function. Like \cite{palm&al18}, it always take the initial hidden state as one of the inputs.
%where $\mcinputfeature(\perm_\query[\ctr]))$ is the initial node feature. 
Notice that the message, $m_t(\valuenode{\ctr})$, is the average of the messages, $\msgfunction_{\redge{}{}}(\rghidden_t(\ctr), \rghidden_t(\ctr_1)) \ \forall \redge{\ctr}{\ctr_1} \in \relationedges$, where $\msgfunction_{\redge{}{}}$ is the message passing function for edge type $\redge{}{}$.
The same function is used during the message passing in $\mcgraph$ for computing messages across edges of type $\redge{}{}$.
The hidden states are updated for $T_R$ steps and the final embeddings, $\rghidden_{T_R}(\valuenode{\ctr}) \ \forall \ctr \in \dspace_k$, are used as `relationship-aware' embeddings for initializing the hidden state of both variable nodes, $\node^\jtr$, and value nodes, $\valuenode{\ctr}$ in the graph $\mcgraph$.

\textbf{Initialization:} 
Initialize the hidden state, $h_0(\valuenode{\ctr})$, for each value node $\valuenode{\ctr}$ in $\mcgraph$, with $\rghidden_{T_R}(\ctr), \ \forall \ctr \in \dspace_k$.
For each variable node $\node^\jtr$, if $\query[\jtr] = \ctr$, then initialize its hidden state, $h_0(\node^\jtr)$, with $\rghidden_{T_R}(\ctr)$.
Otherwise, if $\query[\jtr] = 0$, then initialize $h_0(\node^\jtr)$ with $(1/k)\sum_{
\ctr \in \dspace_k} \rghidden_{T_R}(\ctr)$.

\textbf{Message Passing in $\mcgraph$:}
At time step $t$, similar to \binarymodel, each node receives messages from its neighbors, that are aggregated based on the edge type.
For each node, the aggregated messages, $m_{t,\edgetype{}{}}(\node^\jtr)$, for different edge types, $\edgetype{}{} \in \{\edge{}{}, \redge{}{},  \assignededge{}{}, \naedge{}{} \}$, are stacked to create, $m_t(\node^\jtr)$, which updates the hidden state as:
\begin{equation}
    h_{t+1}(\node^\jtr) = 
    g\left(
    h_t(\node^{\jtr}), m_{t}(\node^{\jtr}),
    h_0(\node^{\jtr})
    \right), \forall \node^{\jtr} \in \mcvertices
\end{equation}


\textbf{Loss Computation and Final Prediction:}
At time step $t$, a scoring function, $\bar{s}$, computes a score for assigning a value $\ctr$ to a variable $\node^\jtr$ based on the hidden state of corresponding value and variable nodes: $\bar{s}_t(\node^\jtr,\valuenode{\ctr}) = s(h_t(\node^\jtr), h_t(\valuenode{\ctr}))$.
For each variable node, a softmax converts these scores into probabilities over the classes $\ctr \in \dspace_k$, \ie, $Pr(\node^\jtr,\ctr) = Softmax(\bar{s}_t(\node^\jtr,\valuenode{\ctr})), \  \forall \ctr \in \dspace_k$.
Total loss at step $t$ is nothing but the average of standard Cross Entropy over variable nodes:
$L_t= - \frac{1}{|\vertices|}\sum_{\node^\jtr \in \vertices} \log(Pr(\node^\jtr, \target[\jtr]))$. 


==> sections/s3b_methods_before_rebuttal.tex <==
\section{Models Description}

\begin{wrapfigure}{r}{0.45\textwidth} 
\vspace{-8ex}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/graphConsExample3.png}
    \caption{An example Futoshiki Puzzle of size $3 \times 3$ and the corresponding graphs. A value of $0$ in the input puzzle represents an unassigned variable. Black and red edges are Constraint and Relation edges respectively.}
    \label{fig:graphexample}
\vspace{-7ex}
\end{wrapfigure}
We propose two models for value-set  invariance: the \emph{\BinaryModel}, and the \emph{\MultiModel}. In each case, we assume the training data
is provided in the form $\traindata=(\{(\query^\itr,G_{C^\itr}),\target^\itr\}_{\itr=1}^{M}, \relationgraph)$ as described in Section~\ref{sec:definition}. %Additionally, we assume 
%we have 
%access to 
Let $\dspace$ and $\testdspace$ denote the value-sets at train and test time, with cardinality $k,k'$, respectively.
%to denote the cardinality of $\dspace$ and $\testdspace$, respectively. 
For each model, we divide the description in the following parts (a) Construction of Message Passing Graph (b) Message Passing Rules (c) Loss Computation, and finally (d) Prediction on a problem with larger value-set.
We describe the details below.

\subsection{Binarized Model}
%\subsubsection{Construction of Message Passing Graph}

\color{blue}
Intuition behind our \BinaryModel\ comes directly from the sparse encoding of an integer CSP into a SAT \cite{kleer89, walsh00}, in which assignment of a value $v \in \dspace$ to any  variable  $\query[\jtr] \in \mathcal{O}$ is encoded by a Boolean variable that represents $\query[\jtr] == v$. 
Such an encoding converts a single multi-valued variable into multiple Boolean valued variables. 
Using sparse encoding, we convert a Constraint Graph (\cref{fig:graphexample}) with nodes representing multi-valued variables (yellow nodes), into a Binary Graph (\cref{fig:graphexample}) with Boolean nodes (blue nodes).
Such a graph can easily represent relationship between the values as well (red edges), thereby encapsulating the information present in the Relation Graph (\cref{fig:graphexample}). We use this Binary Graph for message passing. Below we discuss its construction in detail.
%}

\color{black}
\textbf{Construction of Message Passing Graph:}
We denote the {\em Message Passing Graph (MPG)} by $\bingraph=(\binvertices,\binedges)$ with the set of nodes $\binvertices$ and set of edges $\binedges$, constructed as follows:
{\bf Nodes:} For each node $\node_{\jtr} \in \vertices$ in the Constraint Graph (\cref{fig:graphexample}, yellow nodes), we construct $k$ binary valued nodes, denoted as $\binnode{\jtr}{1},\binnode{\jtr}{2} \cdots \binnode{\jtr}{k}$ in $\binvertices$ (blue nodes in Binary Graph).
Therefore, the total number of nodes constructed is $|\vertices|k$.
{\bf Edges:} We construct two categories of edges in $\bingraph$.
%are divided in two categories described below.\\ \\
%\begin{enumerate}
%\hspace{2ex}{\bf Constraint Edges:} 
The first type of edges are defined for the edges that exist in the constraint graph $\graph$ (black edges). 
For every edge, $\edge{\jtr}{\jtr'} \in \edges$, where $\edge{\jtr}{\jtr'}.type=q$, we introduce $k$ edges denoted as $\binedge{\jtr\ltr}{\jtr'\ltr}$, i.e., there is an edge between every pair of nodes, $\binnode{\jtr}{\ltr}$ and $\binnode{\jtr'}{\ltr}$, $1 \le \ltr \le k$.
These edges are directly inherited from the constraint graph, with $k$ copies created for each edge due to binarization. 
Edge type is same as in the original constraint graph and is denoted by $q$. We refer to these as {\em Constraint Edges}.
We denote the set of all constraint edge types as $Q$.
%{\bf Relational Edges:} 
The second type of edges are defined for relations that exist between values in the value-set. For every pair of binary nodes, $\binnode{\jtr}{\ltr}$ and $\binnode{\jtr}{\ltr'}$, we introduce an edge 
$\binredge{\jtr\ltr}{\jtr\ltr'}$
%$e_{(jl,jl')}^{r}$ 
if 
$\relationfn(v_\ltr,v_{\ltr'})$
%$r(v_l,v_{l'})$ 
holds based on the relationship graph $\relationgraph$, i.e., $\redge{\ltr}{\ltr'} \in \relationedges$ with edge type $r$ (\eg\ red edges encoding  \emph{less-than} relationship between value pairs $(1,2)$, $(2,3)$ and $(1,3)$).
For each relation $r$, there is a total of $|\vertices||r|$ edges introduced in the graph, where $|r|$ denotes the number of (ordered) value pairs from $\dspace$ which are related through $r$. The edge type is the same as the relation $r$. We refer to these as {\em Relational Edges}.
We denote the set of all relational edge types as $R$.

%\subsubsection{Recurrent Message Passing}
\textbf{Recurrent Message Passing:}
\label{subsec:bin_msg}
Once the message passing graph $\bingraph$ has been constructed, we follow message passing rules similar to those used in RRNs~\cite{palm&al18}, with some subtle differences. 
For each node $\binnode{\jtr}{\ltr}$ in the graph, we maintain a hidden state which is updated at each step based on the messages received from its neighbors. 
%Assuming the total of message passing steps as $T$, the final probability of classifying a node (as $0$ or $1$) is computed as $Pr(\binnode{\jtr}{\ltr}.val;\Theta^T)$, where $\Theta^T$ denote the parameters of the model at time step $T$, and $\binnode{\jtr}{\ltr}.val \in \{false,true\}$.

%\bingraph$ is constructed, we run recurrent message passing for some predefined number of steps $T$. At each step, the hidden state of each node, $\binnode{\jtr}{\ltr}$, is updated by the messages received from its neighbors, and finally, based on its hidden state at step $T$, probability, $Pr(\binnode{\jtr}{\ltr} ; \Theta)$, of classifying it as 1 is computed.

\hspace{1ex}\textbf{Initialization:} 
The initial embedding, $\inpfeature(\binnode{\jtr}{\ltr})$, of the nodes $\binnode{\jtr}{\ltr}, \forall v_\ltr$,
is initialized 
%The input features, $\inpfeature(\binnode{\jtr}{\ltr})$, for the nodes $\binnode{\jtr}{\ltr}, \forall \ltr$ are initialized 
based on the initial content of the variable $\query[\jtr], \forall \jtr$.  
If it is unassigned (yellow nodes with $0$ in it), then $\inpfeature(\binnode{\jtr}{\ltr}) = u[-1], \forall v_\ltr \in \dspace$ (\eg\ three blue nodes in the third row of the Binary Graph).
On the other hand, if $\query[\jtr]$ is preassigned a value $v_{\hat{\ltr}}$ (\eg 1st variable assigned a value of `3'), then $\inpfeature(\binnode{\jtr}{\ltr}) = u[0], \forall v_\ltr \neq v_{\hat{\ltr}}$ (\eg\ 1st and 2nd blue nodes in 1st row), and $\inpfeature(\binnode{\jtr}{\hat{\ltr}}) = u[1]$ (\eg\ 3rd blue node in 1st row). 
Here, $u[-1], u[0],$ and $u[1]$ are $3$ learnable embeddings, independent of the size $k$ of the value-set $\dspace$.
The hidden state, $h_0(\binnode{\jtr}{\ltr})$, of each node, $\binnode{\jtr}{\ltr}$, is initialized as a $0$ vector,  $\forall \jtr, \forall v_\ltr$.

\hspace{1ex}\textbf{Edge Dependent Message Passing:}
The nodes communicate their current hidden state via the messages sent to their neighbouring nodes across the edges.
The message depends not only on the current state of the sender and receiver, but also on the \textit{edge type} across which the message is sent. 
Specifically, for each edge type, $\binedgetype{}{}$, there is a separate message passing function,  $\msgfunction_{\binedgetype{}{}}$, with  $\binedgetype{}{} \in (Q \cup R)$ where $Q$ and $R$ are the set of all constraint edge types and relation edge types respectively. We compute the message for each edge $\binedgetype{\jtr_1\ltr_1}{\jtr_2\ltr_2} \in \binedges$ as:
%\begin{equation*}
$
m_t \left[
    \binedgetype{\jtr_1\ltr_1}{\jtr_2\ltr_2}
    \right] =  
    \msgfunction_{\binedgetype{}{}}
    \left(
    h_t \left( \binnode{\jtr_1}{\ltr_1} \right), 
    h_t \left( \binnode{\jtr_2}{\ltr_2} \right)
   \right), 
    \forall 
   \binedgetype{\jtr_1\ltr_1}{\jtr_2\ltr_2} \in \binedges, \ 
   \binedgetype{}{} \in (Q \cup R)  
$.
%\end{equation*}

\hspace{1ex}\textbf{Hidden State Update:}
%Each node maintains its hidden state, $h_t(\binnode{\jtr}{\ltr})$, which is initialized as a `0' vector. 
For each node, the incoming messages on the edges of the same type are aggregated by taking their weighted average. 
The weights, $a_t$, are computed using Bahdanau Attention \cite{bahdanau&al14} over constraint edges, whereas messages across relation edges are simply averaged:
%for constraint edges, whereas messages across $\binredge{}{}$ are simply averaged:
%\begin{equation}
$    m_{t,\binedgetype{}{}}[\binnode{\jtr}{\ltr_1}] =
    \sum_{\binedgetype{\jtr\ltr_1}{\jtr_2\ltr_2} \in \binedges} 
    a_t[\binedgetype{\jtr\ltr_1}{\jtr_2\ltr_2}]
    m_t[\binedgetype{\jtr\ltr_1}{\jtr_2\ltr_2}] \ , \ \forall \binedgetype{}{} \in (Q \cup R) 
$.
%\end{equation}
Finally, all messages, $m_{t,\binedgetype{}{}}[\binnode{\jtr}{\ltr}] \forall \binedgetype{}{} \in (Q \cup R)$, are concatenated to create the input, $m_{t}[\binnode{\jtr}{\ltr}]$ for each node, $\binnode{\jtr}{\ltr}$.
The hidden state at step $t$ is updated by the following state update function to generate the state $h_{t+1}(\binnode{\jtr}{\ltr})$:
%\begin{equation}
$    h_{t+1}(\binnode{\jtr}{\ltr}) = 
    g\left(
    h_t(\binnode{\jtr}{\ltr}), m_{t}[\binnode{\jtr}{\ltr}],
    \inpfeature(\binnode{\jtr}{\ltr})
    \right), \forall \binnode{\jtr}{\ltr} \in \binvertices
$.
%\end{equation}

%\subsubsection{Loss Computation and Prediction}
\textbf{Loss Computation}
%, Target Values and Final Prediction:
%}
At each step $t \in \{1 \ldots T\}$, we can compute the probability $Pr(\binnode{\jtr}{\ltr}.v=1; \Theta)$ of classifying a node $\binnode{\jtr}{\ltr}$ as $1$ by passing its hidden state through a scoring function $s$, \ie,
$Pr_t(\binnode{\jtr}{\ltr}.v=1; \Theta) = \sigma(s(h_t(\binnode{\jtr}{\ltr})))$, where $\sigma$ is the standard Sigmoid function. Here, $\binnode{\jtr}{\ltr}.v$ denotes the value that node $\binnode{\jtr}{\ltr}$ can take and belongs to the set $\{0,1\}$.
The Binary Cross Entropy (BCE) loss for each node $\binnode{\jtr}{\ltr}$ is computed w.r.t. its target, $\bintarget[\jtr,\ltr]$, which is defined as $1$ whenever $\target[\jtr] = \ltr$ and $0$ otherwise.
Total loss at step $t$ is the average BCE loss across all the nodes:
$\frac{1}{|\binvertices|}
\sum\limits_{\binnode{\jtr}{\ltr} \in \binvertices}
\bintarget[\jtr,\ltr] \log Pr_t(\binnode{\jtr}{\ltr}.v=1; \Theta) +
\left(1 - \bintarget[\jtr,\ltr]\right)
\log Pr_t(\binnode{\jtr}{\ltr}.v=0; \Theta)
$.
Like \citet{palm&al18}, we back-propagate through the loss at every step $t \in \{1 \ldots T \}$ as it helps in learning a convergent message passing algorithm. 
%Unlike them, during inference we run message passing till convergence upto a maximum number of steps $T'$.
During training, the objective is to learn the 3 initial embeddings $u[-1], u[0], u[1]$, message passing functions $\msgfunction_{\binedgetype{}{}}, \forall \binedgetype{}{} \in Q \cup R$, attention function $a$, state update function $g$, and the scoring function $s$.

\noindent \textbf{Prediction on a problem with larger size of value-set:}
While testing, let the constraint and relation graph be $\testgraph$ and $\testrelationgraph$ with $n'$ and $k'$ nodes respectively. Let $\testquery$ be a partial solution, with $n'$ variables $\testquery[\jtr]$, each taking a value from value-set $\testdspace$ of size $k'$.
As described above, we create a graph $\bingraph'$ with $n'k'$ nodes, run message passing for $T$ steps, and for each variable $\testquery[\jtr]$, compute the $k'$ probabilities, one for each of the $k'$ nodes
 $\binnode{\jtr}{\ltr} \forall \ltr \in \testdspace$ corresponding to the variable $\testquery[\jtr]$, which is assigned the value corresponding to maximum probability, \ie, $\pred[\jtr] = \argmax_{\ltr \in \testdspace} Pr_{T}(\binnode{\jtr}{\ltr}.v=1 ; \Theta) $.

\subsection{Multi-valued Model}
%Augmenting the Multi-class Classification: \multimodel }
%We next introduce the \multimodel. 
%To achieve domain size invariance in this method, we introduce $k$ new nodes of a different type in the original primal constraint graph $\graph$.
%Each new node corresponds to a class in $\dspace$.
%To distinguish them from the variable nodes, we call them \textit{value nodes}.
%Notice that it makes the new graph heterogeneous not only w.r.t. edges, but also w.r.t. nodes, unlike the graph $\bingraph$ in \binarymodel.
%After message passing, each variable node is classified by computing a bi-linear similarity score between its hidden state and the hidden state of each of the value nodes. 
%It is assigned the class represented by the value node corresponding to the maximum similarity score. 
%\subsubsection{Construction of Message Passing Graph}
\textbf{Construction of Message Passing Graph(s):}
Multi-valued model differs from the \binarymodel\ by avoiding binarization of nodes, and instead explicitly adding nodes in the message passing graph, one for each value in the value-set. The message graph consists of two components: (a) A Graph $\mvgraph=(\mvvertices,\mvedges)$ to represent constraints inherited from the constraint graph $\graph=(\vertices,\edges)$ (b) A Graph $\mvrgraph=(\mvrvertices,\mvredges)$ to represent relations inherited from the relationship graph $\relationgraph=(\relationvertices,\relationedges)$. We refer to $\mvgraph$ as {\em Constraint Message Passing Graph}, and $\mvrgraph$ as {\em Relationship Message Passing Graph}. %We describe the construction for each of them next.

\noindent {\bf Construction of Constraint Message-Passing Graph (CMPG)}
%: $\mvgraph(\mvvertices,\mvedges)$} 

\hspace{1ex}{\bf Nodes:} For each node $\node_{\jtr} \in \vertices$ in the constraint graph, we construct a $k$-valued node, denoted as $\mvnode{\jtr} \in \mvvertices$. Total number of such nodes constructed is $|\vertices|$. We refer to these as {\em Variable Nodes} (yellow nodes in Multi-Valued Graph in \cref{fig:graphexample}). 
Additionally, for each value $v_\ltr \in \dspace$ in the value-set, we create a node, denoted as 
$\mvvalnode{\ltr} \in \mvvertices$. Total number of such nodes constructed is $|\dspace|$.
We refer to these as {\em Value Nodes} (orange nodes).
\hspace{1ex}{\bf Edges:} 
%There is a one to one correspondence of these edges to those present in the constraint graph. 
For every edge, $\edge{\jtr}{\jtr'} \in \edges$, where $\edge{\jtr}{\jtr'}.type=q$, we introduce an edge denoted as $\mvedge{\jtr}{\jtr'}$ with type $q$. These edges are directly inherited from the constraint graph. Edge type is same as in the original constraint graph and is denoted by $q$. 
We refer to these as {\em Constraint Edges} (black edges) 
and 
%We denote 
the set of all constraint edge types as $Q$.
Additionally, to indicate the pre-assignment of values to the variables in $\query$, we introduce new edges connecting value nodes to appropriate  variable nodes.
Whenever $\query[\jtr]=v_\ltr$, add an edge, $\mvaedge{\jtr}{\ltr}$ between variable node $\mvnode{\jtr}$ and value node $\mvvalnode{\ltr}$ (blue edges).
If $\query[\jtr]$ is \mask, \ie, unassigned, then add $k$ edges, $\mvuaedge{\jtr}{\ltr}, \forall v_\ltr \in \dspace$, connecting the variable node $\mvnode{j}$ with all $k$ value nodes $\mvvalnode{\ltr}$ (\eg, green edges connecting orange value node `2' to all `0' yellow variable nodes).
We refer to them as {\em assignment edges}.
%, and denote the set of their types by $A$. 
%We denote the set of all assignment edge types as $A$.

\noindent {\bf Construction of Relationship Message-Passing Graph (RMPG)}
%: $\mvrgraph(\mvrvertices, \mvredges)$} 

\hspace{1ex}{\bf Nodes:} For each value 
$v_\ltr \in \dspace$,
%in the value-set,
create a node denoted as $\mvrvalnode{\ltr} \in \mvrvertices$ (purple nodes in Relation Graph in \cref{fig:graphexample}). Total number of such nodes constructed is $|\dspace|$. We refer to these as {\em Value Nodes}. 
%These value nodes are distinct from those introduced in CPMG.
\hspace{1ex}{\bf Edges:} For every pair of value nodes, 
$\mvrvalnode{\ltr}$
and 
$\mvrvalnode{\ltr'}$, 
introduce an edge $\mvrredge{\ltr}{\ltr'}$ if $\relationfn(v_\ltr,v_{\ltr'})$ holds based on the relationship graph $\relationgraph$, i.e.,
$\redge{\ltr}{\ltr'} \in \relationedges$ with edge label $r$ (red edges). 
The edge type is the same as relation $r$.
These types of edges are defined for relations that exist between values in the value-set and
we refer to them as {\em Relational Edges} and denote the set of all relational edge types as $R$.

%\subsubsection{Achieving Domain-size Invariance}
\textbf{Achieving Value-set Invariance:}
A key question arises here: why do we need to construct a separate RMPG ($\tilde{G})$? Why not embed relevant edges in CMPG ($G$), as done for the \binarymodel? The answer lies in realizing that we represent each value in the value-set explicitly in the \multimodel, unlike the \binarymodel.  Hence, our model needs to learn representation for each of them in the form of value node embeddings. 
Further, to generalize we need to learn as many embeddings as there are values in the largest test value-set, i.e., $k_{\max}=\max |\mathcal{V}'|$.
We achieve this by randomly sub-selecting a $k$-sized set from $\{1\ldots k_{\max}\}$ and permuting the chosen subset for each training example in a given mini-batch, and then computing the `relationship-aware' embeddings from this permuted subset through message passing in RMPG.
%(Relation Graph in \cref{fig:graphexample}). 
The `relationship-aware' embeddings are then used to initialize the value nodes (orange nodes) during message passing in CMPG. 
For instance, if the permutation obtained is 
$\{w_1,\cdots,w_\ltr,\cdots,w_k\}$, where  $\forall \ltr, 1 \le w_\ltr \le k_{\max}$, 
then embedding for the
value node $\mvrvalnode{\ltr}$ in $\mvrgraph$ is initialized by $w_\ltr^{th}$ learnable embedding (\eg, purple nodes for values `1', `2', and `3' are initialized by the 5th, 7th, and 1st learnable embedding, respectively).
After message passing on $\mvrgraph$, the `relationship-aware' embedding of $\mvrvalnode{\ltr}$ (purple node) is used to initialize the embedding for
value node $\mvvalnode{\ltr}$ (orange node) in $\mvgraph$.
%is initialized with $w_\ltr^{th}$ relationship-aware embedding. 
This elegant process is able to train all the $k_{\max}$ embeddings by simply using the training data corresponding to
$\mathcal{V}$,
and the corresponding relationship information. 
Since these relationship aware embeddings need to be pre-computed before they can be passed to the downstream constraint processing, we construct two different message passing graphs, one for computing relationship-aware embeddings and one for constraint handling. 
%We note that \binarymodel\ circumvents this issue by
%We note that parameters associated with message-passing 

\begin{comment}
set of $k$ values from the test domain size $\mathcal{V}'$, 
computing the \ycom{`relationship aware'} embeddings for each of them, and then enforcing the constraints.~\footnote{we assume $k' \ge k $, the other case is trivially handled.} 
\ycom{this is not correct. We are not selecting $k$ values from test domain size $\dspace'$. Instead, for an RMPG with $k$ value nodes, we are randomly selecting any $k$ out of $k'$ learnable embeddings to initialize them. Since we have $k'$ learnable permutation invariant embeddings, we can work with RMPG with upto $k'$ value nodes.}
Since, the embeddings constructed should obey the relationships between values in the domain, they are constructed by first passing messages over RMPG which represents relationships. This is followed by message passing in CMPG to enforce constraints. Having two separate graphs for the two allows our model to perform these steps sequentially, one after another, in a single joint model. Therefore, when constraints are enforced, we have stable value embeddings which we can work with; having them updated during constraint processing led to poor generalization. As a result, our model can learn value embeddings for an unseen domain $\mathcal{V}'$, while only using the training data for a completely different domain $\mathcal{V}$, as long as the relationship information for the two is available at test and train times, respectively. This is precisely the reason our \multimodel\ can achieve domain-size invariance. This issue does not arise in binary model, since it does away with the need to represent different values by binarizing all of them, and thus learning the embeddings for two fixed constants `0' and `1'. Later in this section, we present some discussion on relative (theoretical) merit of our two proposed models.
\end{comment}

%\subsubsection{Recurrent Message Passing (RMPG)}
\textbf{Recurrent Message Passing on RMPG}

\hspace{1ex}\textbf{Initialization:} For each query $\query$, select a $k-$permutation, $\perm_\query$, of $k_{\max}$ (\eg, $(5,7,1)$, shown in square boxes in \cref{fig:graphexample}).
Initialize the embedding of $\mvrvalnode{\ltr}$ (purple nodes) in  $\mvrgraph$ with $\mvrinputfeature[\perm_\query[\ltr]], \ \forall \ltr \in \{1 \ldots k\}$ (\eg, $\mvrinputfeature[5], \mvrinputfeature[7], \mvrinputfeature[1] $ for initializing purple value nodes `1',`2', and `3' respectively).
Here, $\mvrinputfeature[\ltr'], \ltr' \in \{1 \ldots k_{\max}\}$, are $k_{\max}$ learnable embeddings.
Initialize the hidden state, $\rghidden_0(\mvrvalnode{\ltr}), \ \forall \mvrvalnode{\ltr} \in \mvrvertices$ with a $0$ vector. 
%We randomly select any $k$ out of $k'$ learnable embeddings to initialize the $k$ value nodes $\mvrvalnode{\ltr}, \forall \ltr \in \dspace$ in $\mvrgraph$.
%To achieve domain size invariance upto domain size $k_{max}$, we keep  $k_{max}$ learnable input features: $\mcinputfeature(\ltr) \  \forall \ltr \in \{1 \ldots k_{max} \}$. 
%\textbf{Input Features: } 
Computation of messages and hidden state update at step $t$ is similar to the one described for \BinaryModel\ in \cref{subsec:bin_msg}.
Exact equations are in the appendix. 
Hidden states are updated for $\tilde{T}$ steps and the final embeddings, $\rghidden_{\tilde{T}}(\mvrvalnode{\ltr}) \ \forall v_\ltr \in \dspace$, are used as `relationship-aware' embeddings for initializing the input features (embeddings) of the nodes in CMPG $\mvgraph$.
%both variable nodes, $\mvnode{\jtr}$, and value nodes, $\mvvalnode{\ltr}$ in $\mvgraph$ (orange and yellow nodes respectively in Multi-valued Graph).

%\subsubsection{Recurrent Message Passing (CMPG)}
\textbf{Recurrent Message Passing on CMPG}

\hspace{1ex}\textbf{Initialization:} Initialize the embedding of value nodes (orange nodes), $\mvvalnode{\ltr}$ in $\mvgraph$, using the  final `relationship-aware' embeddings, $\rghidden_{\tilde{T}}(\mvrvalnode{\ltr})$, of $\mvrvalnode{\ltr}$ (purple nodes) in $\mvrgraph$.
The variable nodes that are preassigned a value (non-zero yellow nodes) in $\query$, are initialized by the embedding of the corresponding value node, \ie, if $\query[\jtr] = \ltr$, then $\mvnode{\jtr}$ is initialized with the `relationship-aware' embedding, $\rghidden_{\tilde{T}}(\mvrvalnode{\ltr})$, of $\mvrvalnode{\ltr}$.
On the other hand, the embedding of nodes corresponding to the unassigned variables (`0' yellow nodes) are initialized by the average, $(1/k)\sum_{
v_\ltr \in \dspace} \rghidden_{\tilde{T}}(\mvrvalnode{\ltr})$, of all `relationship-aware' embeddings.
For a variable node $\mvnode{\jtr}$, we denote its initial embedding as:
$\inpfeature(\mvnode{\jtr})$.
Initialize the hidden state, $h_0(\mvnode{\jtr})$, for each variable node $\mvnode{\jtr}$ in $\mvgraph$, with
a $0$ vector.
Message passing and state update is similar to the one described for \BinaryModel. See appendix for details.

\textbf{Loss Computation:}
At step $t$, a scoring function, $s$, computes a score, $s(h_t(\mvnode{\jtr}), h_t(\mvvalnode{\ltr}))$,  for assigning a value $v_\ltr$ to a variable $\mvnode{\jtr}$ based on the hidden state of corresponding value and variable nodes.
For each variable node, a $Softmax$ converts these scores into probabilities over the values $v_\ltr \in \dspace$, \ie, $Pr(\mvnode{\jtr}.v = v_\ltr) = Softmax(s(h_t(\mvnode{\jtr}), h_t(\mvvalnode{\ltr}))), \  \forall v_\ltr \in \dspace$, 
where, $\mvnode{\jtr}.v \in \dspace$ denotes the value that node $\mvnode{\jtr}$ can take.
Total loss at step $t$ is nothing but the average of standard Cross Entropy over variable nodes:
$L_t= - \frac{1}{|\mvvertices|}\sum_{\mvnode{\jtr} \in \mvvertices} \log Pr(\mvnode{\jtr}.v= \target[\jtr])$. 
To ensure that the \multimodel\ learns different embeddings for each value in the value-set, we add an auxiliary loss term, corresponding to the total pairwise dot product (similarity) of any two embeddings, before and after message passing in
$\mvrgraph$. 
We call it \emph{Orthogonality Loss}. Its weight, $\alpha$, is a hyper-parameter.

\textbf{Prediction on a problem with larger size of value-set:}
For a puzzle with larger value-set, $\testdspace$, a bigger RMPG is created, whose $k'$ nodes are initialized with the (learnt) first $k'$ embeddings. 
Unlike training, we always choose first $k'$ embeddings to avoid randomness during testing.
Prediction is made using the probabilities at the last step $T$, \ie, $\pred[\jtr] = \argmax_{v_\ltr \in \testdspace} Pr(\mvnode{\jtr}.v = v_\ltr)$.

\textbf{Relative Comparison:}
%Drawbacks of \binarymodel}
In the \binarymodel, the constructed graph $\bingraph$ has $k|\vertices|$ nodes and at least $k|\edges| +  |\vertices|k(k-1)/2$ edges due to binarization. This increases the graph size by a factor of at least $k$. As a result, we soon hit the memory limits of a GPU while training the \binarymodel\ with bigger problems. The model also needs significantly more inference time due to its bigger size. On the other hand, \multimodel, while being compact in terms of its representation, needs to learn additional embeddings, for a speculative size of value-set during testing. 
This poses additional requirement on the model both in terms of representation, and learning, possibly affecting the quality of generalization. While this is a simple analytical understanding of the possible merits of the two models, we examine experimentally the impact of these issues on real datasets. 
%This is presented in the next section.

==> sections/s3b_methods_withsubsubsections.tex <==
\begin{comment}
\begin{figure}[h!]
  \centering
  \begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{figures/train-pipeline.jpg}
    \caption{Train pipeline}
  \end{subfigure} 
  \hspace{0.1\textwidth}
  \begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{figures/test-pipeline.jpg}
    \caption{Test pipeline}
  \end{subfigure}
  \caption{Pipeline for domain-invariance}
  \label{fig:domain-inv-pipeline}
\end{figure}
\end{comment}


\section{Models Description}
We propose two models for domain-size invariance, \ie, the \binarymodel\ , and the \multimodel. In each case, we assume the training data
is provided in the form $\traindata=(\{\query^\itr,\target^\itr\}_{\itr=1}^{m}, \graph,\relationgraph)$ as described in Section~\ref{sec:definition}. 
Additionally, we assume 
%we have 
access to $\dspace$ and $\testdspace$, i.e., domains at train and test time, respectively. We will use $k,k'$ to denote the cardinality of $\dspace$ and $\testdspace$, respectively. 
For each model, we divide the description in the following parts (a) Construction of Message Passing Graph (b) Message Passing Rules and (c) Loss Computation. 
We describe the details below.


\subsection{Binary Model}
\subsubsection{Construction of Message Passing Graph}
We denote the {\em Message Passing Graph (MPG)} by $\bingraph=(\binvertices,\binedges)$ with the set of nodes $\binvertices$ and set of edges $\binedges$.  \\ \\
%We refer to this graph as {\em Message Passing Graph (MPG)}.\\ \\
%as described below. \\
{\bf Nodes:} For each node $\node_{\jtr} \in \vertices$ in the constraint graph, we construct $k$ binary valued nodes, denoted as $\binnode{\jtr}{1},\binnode{\jtr}{2} \cdots \binnode{\jtr}{k}$ in $\binvertices$. 
Therefore, the total number of nodes constructed is $|\vertices|k$. \\ \\
{\bf Edges:} We construct two categories of edges in $\bingraph$.
%are divided in two categories described below.\\ \\
%\begin{enumerate}
%\hspace{2ex}{\bf Constraint Edges:} 
The first type of edges are defined for the edges that exist in the constraint graph $\graph$. 
For every edge, $\edge{\jtr}{\jtr'} \in \edges$, where $\edge{\jtr}{\jtr'}.type=q$, we introduce $k$ edges denoted as $\binedge{\jtr\ltr}{\jtr'\ltr}$, i.e., there is an edge between every pair of nodes, $\binnode{\jtr}{\ltr}$ and $\binnode{\jtr'}{\ltr}$, $1 \le \ltr \le k$.
These edges are directly inherited from the constraint graph, with $k$ copies created for each edge due to binarization. 
Edge type is same as in the original constraint graph and is denoted by $q$. We refer to these as {\em Constraint Edges}.
We denote the set of all constraint edge types as $Q$.
%{\bf Relational Edges:} 
The second type of edges are defined for relations that exist between values in the domain. For every pair of binary nodes, $\binnode{\jtr}{\ltr}$ and $\binnode{\jtr}{\ltr'}$, we introduce an edge 
$\binredge{\jtr\ltr}{\jtr\ltr'}$
%$e_{(jl,jl')}^{r}$ 
if 
$\relationfn(v_\ltr,v_{\ltr'})$
%$r(v_l,v_{l'})$ 
holds based on the relationship graph $\relationgraph$, i.e., $\redge{\ltr}{\ltr'} \in \relationedges$ with edge type $r$. 
For each relation $r$, there is a total of $|\vertices||r|$ edges introduced in the graph, where $|r|$ denotes the number of (ordered) value pairs from $\dspace$ which are related through $r$. The edge type is the same as the relation $r$. We refer to these as {\em Relational Edges}.
We denote the set of all relational edge types as $R$.

\subsubsection{Recurrent Message Passing}\label{subsec:bin_msg}
Once the message passing graph $\bingraph$ has been constructed, we follow message passing rules similar to those used in RRNs~\cite{palm&al18}, with some subtle differences. 
For each node $\binnode{\jtr}{\ltr}$ in the graph, we maintain a hidden state which is updated at each step based on the messages received from its neighbors. 
%Assuming the total of message passing steps as $T$, the final probability of classifying a node (as $0$ or $1$) is computed as $Pr(\binnode{\jtr}{\ltr}.val;\Theta^T)$, where $\Theta^T$ denote the parameters of the model at time step $T$, and $\binnode{\jtr}{\ltr}.val \in \{false,true\}$.

%\bingraph$ is constructed, we run recurrent message passing for some predefined number of steps $T$. At each step, the hidden state of each node, $\binnode{\jtr}{\ltr}$, is updated by the messages received from its neighbors, and finally, based on its hidden state at step $T$, probability, $Pr(\binnode{\jtr}{\ltr} ; \Theta)$, of classifying it as 1 is computed.

\textbf{Initialization:} 

The initial embedding, $\inpfeature(\binnode{\jtr}{\ltr})$, of the nodes, $\binnode{\jtr}{\ltr}, \forall v_\ltr$,
is initialized 
%The input features, $\inpfeature(\binnode{\jtr}{\ltr})$, for the nodes $\binnode{\jtr}{\ltr}, \forall \ltr$ are initialized 
based on the initial content of the variable $\query[\jtr], \forall \jtr$.  
If it is \mask, \ie unassigned, then $\inpfeature(\binnode{\jtr}{\ltr}) = u[-1], \forall v_\ltr \in \dspace$.
On the other hand, if $\query[\jtr]$ is preassigned a value $v_{\hat{\ltr}}$, then $\inpfeature(\binnode{\jtr}{\ltr}) = u[0], \forall v_\ltr \neq v_{\hat{\ltr}}$, and $\inpfeature(\binnode{\jtr}{\hat{\ltr}}) = u[1]$. 
Here, $u[-1], u[0], u[1]$ are $3$ learnable embeddings.
The hidden state, $h_0(\binnode{\jtr}{\ltr})$, of each node, $\binnode{\jtr}{\ltr}$, is initialized as a `0' vector,  $\forall \jtr, \forall v_\ltr$.

\textbf{Edge Dependent Message Passing:}
The nodes communicate their current hidden state via the messages sent to their neighbouring nodes across the edges.
The message depends not only on the current state of the sender and receiver, but also on the \textit{edge type} across which the message is sent. 
Specifically, for each edge type, $\binedgetype{}{}$, there is a separate message passing function,  $\msgfunction_{\binedgetype{}{}}$, with  $\binedgetype{}{} \in (Q \cup R)$ where $Q$ and $R$ are the set of all constraint edge types and relation edge types respectively. We compute the message for each edge $\binedgetype{\jtr_1\ltr_1}{\jtr_2\ltr_2} \in \binedges$ as:

\begin{equation}
m_t \left(
    \binedgetype{\jtr_1\ltr_1}{\jtr_2\ltr_2}
    \right) =  
    \msgfunction_{\binedgetype{}{}}
    \left(
    h_t \left( \binnode{\jtr_1}{\ltr_1} \right), 
    h_t \left( \binnode{\jtr_2}{\ltr_2} \right)
   \right), 
    \forall 
   \binedgetype{\jtr_1\ltr_1}{\jtr_2\ltr_2} \in \binedges, \ 
   \binedgetype{}{} \in (Q \cup R)  
\end{equation}

\textbf{Hidden State Update:}
%Each node maintains its hidden state, $h_t(\binnode{\jtr}{\ltr})$, which is initialized as a `0' vector. 
For each node, the incoming messages on the edges of the same type are aggregated by taking their weighted average. 
The weights, $a_t$, are computed using Bahdanau Attention \cite{bahdanau&al14} over constraint edges, whereas messages across relation edges are simply averaged:
%for constraint edges, whereas messages across $\binredge{}{}$ are simply averaged:

\begin{equation}
    m_{t,\binedgetype{}{}}(\binnode{\jtr}{\ltr_1}) =
    \sum\limits_{\binedgetype{\jtr\ltr_1}{\jtr_2\ltr_2} \in \binedges} 
    a_t(\binedgetype{\jtr\ltr_1}{\jtr_2\ltr_2})
    m_t(\binedgetype{\jtr\ltr_1}{\jtr_2\ltr_2}) \ , \ \forall \binedgetype{}{} \in (Q \cup R) 
\end{equation}

Finally, all messages, $m_{t,\binedgetype{}{}}(\binnode{\jtr}{\ltr}) \forall \binedgetype{}{} \in (Q \cup R)$, are concatenated to create the input, $m_{t}(\binnode{\jtr}{\ltr})$ for each node, $\binnode{\jtr}{\ltr}$.
The hidden state at time step $t$ is updated by the following state update function to generate the state $h_{t+1}(\binnode{\jtr}{\ltr})$:
\begin{equation}
    h_{t+1}(\binnode{\jtr}{\ltr}) = 
    g\left(
    h_t(\binnode{\jtr}{\ltr}), m_{t}(\binnode{\jtr}{\ltr}),
    \inpfeature(\binnode{\jtr}{\ltr})
    \right), \forall \binnode{\jtr}{\ltr} \in \binvertices
\end{equation}

\subsubsection{Loss Computation and Prediction}
%, Target Values and Final Prediction: 
%}
At each step $t \in {1 \ldots T}$, we can compute the probability $Pr(\binnode{\jtr}{\ltr}.v=1; \Theta)$ of classifying a node $\binnode{\jtr}{\ltr}$ as $1$ by passing its hidden state through a scoring function $s$, \ie,
$Pr_t(\binnode{\jtr}{\ltr}.v=1; \Theta) = \sigma(s(h_t(\binnode{\jtr}{\ltr})))$, where $\sigma$ is the standard Sigmoid function. Here, $\binnode{\jtr}{\ltr}.v$ denotes the value that node $\binnode{\jtr}{\ltr}$ can take and belongs to the set $\{0,1\}$.

The Binary Cross Entropy (BCE) loss for each node $\binnode{\jtr}{\ltr}$ is computed w.r.t. its target, $\bintarget[\jtr,\ltr]$, which is defined as $1$ whenever $\target[\jtr] = \ltr$ and $0$ otherwise.
Total loss at time step $t$ is the average BCE loss across all the nodes:
%\\
%\vspace{0.5ex}
$\frac{1}{|\binvertices|}
\sum\limits_{\binnode{\jtr}{\ltr} \in \binvertices}
\bintarget[\jtr,\ltr] \log Pr_t(\binnode{\jtr}{\ltr}.v=1; \Theta) +
\left(1 - \bintarget[\jtr,\ltr]\right)
\log Pr_t(\binnode{\jtr}{\ltr}.v=0; \Theta)
$
\begin{comment}
\begin{equation}
    \totalloss_t = \frac{1}{|\binvertices|}
    \sum\limits_{\binnode{\jtr}{\ltr} \in \binvertices}
    \bintarget[\jtr,\ltr] \log Pr_t(\binnode{\jtr}{\ltr}.v=1; \Theta) +
    \left(1 - \bintarget[\jtr,\ltr]\right)
    \log Pr_t(\binnode{\jtr}{\ltr}.v=0; \Theta)
\end{equation}
\end{comment}

Like \citet{palm&al18}, while training we back-propagate through the loss at every time step $t \in \{1 \ldots T \}$ as it helps in learning a convergent message passing algorithm. 
%Unlike them, during inference we run message passing till convergence upto a maximum number of steps $T'$.

Finally, %for each original variable, $\node^\jtr$, 
we compare the $k$ probabilities for $\binnode{\jtr}{\ltr} \forall \ltr \in \dspace$, and assign it the value corresponding to maximum probability, \ie, $\pred[\jtr] = \argmax_{\ltr \in \dspace} Pr_{T}(\binnode{\jtr}{\ltr} ; \Theta) $.
\begin{comment}
\begin{figure}[h!]
  \centering
  \begin{subfigure}[b]{0.1\linewidth}
    \includegraphics[width=\linewidth]{figures/Puzzle-eg.jpg}
    \caption{Query}
  \end{subfigure} 
  \hspace{0.1\textwidth}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{figures/Binary.jpg}
    \caption{Binary Graph}
  \end{subfigure}
  \hspace{0.1\textwidth}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{figures/Multi-Value.jpg}
    \caption{Multi-Value Graph}
  \end{subfigure} 
  \caption{Graph Construction}
  \label{fig:domain-inv-pipeline}
\end{figure}
\end{comment}

\subsection{Multi-valued Model}
%Augmenting the Multi-class Classification: \multimodel }
%We next introduce the \multimodel. 
%To achieve domain size invariance in this method, we introduce $k$ new nodes of a different type in the original primal constraint graph $\graph$.
%Each new node corresponds to a class in $\dspace$.
%To distinguish them from the variable nodes, we call them \textit{value nodes}.
%Notice that it makes the new graph heterogeneous not only w.r.t. edges, but also w.r.t. nodes, unlike the graph $\bingraph$ in \binarymodel.
%After message passing, each variable node is classified by computing a bi-linear similarity score between its hidden state and the hidden state of each of the value nodes. 
%It is assigned the class represented by the value node corresponding to the maximum similarity score. 

\subsubsection{Construction of Message Passing Graph}
Multi-valued model differs from the \binarymodel\ by avoiding binarization of nodes, and instead making each node in the message passing graph represent each value in the domain explicitly. The message graph consists of two components: (a) A Graph $\mvgraph=(\mvvertices,\mvedges)$ to represent constraints inherited from the constraint graph $\graph=(\vertices,\edges)$ (b) A Graph $\mvrgraph=(\mvrvertices,\mvredges)$ to represent relationships inherited from the relationships graph $\relationgraph=(\relationvertices,\relationedges)$. We refer to $\graph$ as the {\em Constraint Message Passing Graph}, and $\mvgraph$ as {\em Relationship Message Passing Graph}. We describe the construction for each of them next.

\noindent {\bf Construction of $\mvgraph(\mvvertices,\mvedges)$:} Constraint Message-Passing Graph (CMPG)

{\bf Nodes:} For each node $\node_{\jtr} \in \vertices$ in the constraint graph, we construct a $k$-valued node, denoted as $\mvnode{\jtr} \in \mvvertices$. Total number of such nodes constructed is $|\vertices|$. We refer to these as {\em Variable Nodes}. 
Additionally, for each value $v_\ltr \in \dspace$ in the domain, we create a node, denoted as 
$\mvvalnode{\ltr} \in \mvvertices$. Total number of such nodes constructed is $|\dspace|$.
We refer to these as {\em Value Nodes}. \\

{\bf Edges:} There is a one to one correspondence of these edges to those present in the constraint graph. For every edge, $\edge{\jtr}{\jtr'} \in \edges$, where $\edge{\jtr}{\jtr'}.type=q$, we introduce an edge denoted as $\mvedge{\jtr}{\jtr'}$ with type $q$. These edges are directly inherited from the constraint graph. Edge type is same as in the original constraint graph and is denoted by $q$. We refer to these as {\em Constraint Edges}. We denote the set of all constraint edge types as $Q$.
Additionally, to indicate the pre-assignment of values to the variables in $\query$, we introduce new edges connecting value nodes to appropriate  variable nodes.
Whenever $\query[\jtr]=v_\ltr$, add an edge, $\mvaedge{\jtr}{\ltr}$ between variable node $\mvnode{\jtr}$ and value node $\mvvalnode{\ltr}$.
If $\query[\jtr]$ is \mask, \ie, unassigned, then add $k$ edges, $\mvuaedge{\jtr}{\ltr}, \forall v_\ltr \in \dspace$, connecting the variable node $\mvnode{j}$ with all $k$ value nodes $\mvvalnode{\ltr}$.
We refer to them as {\em assignment edges}. We denote the set of all assignment edge types as $A$.
\\

\noindent {\bf Construction of $\mvrgraph(\mvrvertices, \mvredges):$} Relationship Message-Passing Graph (RMPG)

{\bf Nodes:} For each value 
$v_\ltr \in \dspace$ 
%$v \in \mathcal{V}$ 
in the domain, create a node denoted as $\mvrvalnode{\ltr} \in \mvrvertices$. Total number of such nodes constructed is $|\dspace|$. We refer to these as {\em Value Nodes}. These value nodes are distinct from those introduced in CPMG.
%\ycom{we used value nodes in CMPG as well}. 

{\bf Edges:} These types of edges are defined for relations that exist between values in the domain. For every pair of value nodes, 
$\mvrvalnode{\ltr}$, 
and 
$\mvrvalnode{\ltr'}$, 
we introduce an edge $\mvrredge{\ltr}{\ltr'}$ if $\relationfn(v_\ltr,v_{\ltr'})$ holds based on the relationship graph $\relationgraph$, i.e.,
$\redge{\ltr}{\ltr'} \in \relationedges$ with edge label $r$. 
The edge type is the same as the relation $r$. We refer to these as {\em Relational Edges}. We denote the set of all relational edge types as $R$.

\subsubsection{Achieving Domain-size Invariance}
A key question arises here: why do we need to construct a separate RMPG ($\tilde{G})$, why not embed relevant edges in CMPG ($G$), as done for the \binarymodel. The answer lies in realizing that in the \multimodel\ , we are representing each value in the domain explicitly, unlike in the \binarymodel\ .  Hence, our model needs to learn representation for each of them in the form of value node embeddings. Further, we need to be able to learn as many embeddings as there are values in $\max$ test domain size, i.e., $k_{\max}=\max |\mathcal{V}'|$, in order to be able to generalize. We achieve this by randomly sub-selecting a $k$-sized set from $\{1\ldots k_{\max}\}$ and permuting the chosen subset, for each training example in a given mini-batch, and then, computing the `relationship-aware' embeddings for this permuted subset through message passing in RMPG. The `relationship-aware' embeddings are then used to initialize the value nodes during message passing in CMPG. For instance, if the permutation obtained is 
$\{w_1,\cdots,w_\ltr,\cdots,w_k\}$, where for $\forall \ltr, 1 \le w_\ltr \le k_{\max}$, 
then embedding for the
value node $\mvrvalnode{\ltr}$ in $\mvrgraph$ is initialized by $w_\ltr^{th}$ learnable embedding, and after message passing on $\mvrgraph$, the `relationship-aware' embedding of $\mvrvalnode{\ltr}$ is used to initialize the embedding for
value node $\mvvalnode{\ltr}$ in $\mvgraph$.
%is initialized with $w_\ltr^{th}$ relationship-aware embedding. 
This elegant process is able to train all the $k_{\max}$ embeddings by simply using the training data corresponding to
$\mathcal{V}$,
and the corresponding relationship information. Since these relationship aware embeddings needs to be pre-computed before they can be passed to the downstream constraint processing, we construct two different message passing graphs, one for computing relationship-aware embeddings, and then, for constraint handling. 
%We note that \binarymodel\ circumvents this issue by
%We note that parameters associated with message-passing 

\begin{comment}
set of $k$ values from the test domain size $\mathcal{V}'$, 
computing the \ycom{`relationship aware'} embeddings for each of them, and then enforcing the constraints.~\footnote{we assume $k' \ge k $, the other case is trivially handled.} 
\ycom{this is not correct. We are not selecting $k$ values from test domain size $\dspace'$. Instead, for an RMPG with $k$ value nodes, we are randomly selecting any $k$ out of $k'$ learnable embeddings to initialize them. Since we have $k'$ learnable permutation invariant embeddings, we can work with RMPG with upto $k'$ value nodes.}
Since, the embeddings constructed should obey the relationships between values in the domain, they are constructed by first passing messages over RMPG which represents relationships. This is followed by message passing in CMPG to enforce constraints. Having two separate graphs for the two allows our model to perform these steps sequentially, one after another, in a single joint model. Therefore, when constraints are enforced, we have stable value embeddings which we can work with; having them updated during constraint processing led to poor generalization. As a result, our model can learn value embeddings for an unseen domain $\mathcal{V}'$, while only using the training data for a completely different domain $\mathcal{V}$, as long as the relationship information for the two is available at test and train times, respectively. This is precisely the reason our \multimodel\ can achieve domain-size invariance. This issue does not arise in binary model, since it does away with the need to represent different values by binarizing all of them, and thus learning the embeddings for two fixed constants `0' and `1'. Later in this section, we present some discussion on relative (theoretical) merit of our two proposed models.
\end{comment}

\subsubsection{Recurrent Message Passing (RMPG)}
\textbf{Initialization:} 
For each query $\query$, select a $k-$permutation, $\perm_\query$, of $k_{\max}$.
Initialize the embedding of $\mvrvalnode{\ltr}$ in  $\mvrgraph$ with $\mvrinputfeature(\perm_\query[\ltr]), \ \forall \ltr \in \{1 \ldots k\}$.
Here, $\mvrinputfeature[\ltr'], \ltr' \in {1 \ldots k_{\max}}$, are $k_{\max}$ learnable embeddings.
Initialize the hidden state, $\rghidden_0(\mvrvalnode{\ltr}), \ \forall \mvrvalnode{\ltr} \in \mvrvertices$ with a $0$ vector. 

%We randomly select any $k$ out of $k'$ learnable embeddings to initialize the $k$ value nodes $\mvrvalnode{\ltr}, \forall \ltr \in \dspace$ in $\mvrgraph$.
%To achieve domain size invariance upto domain size $k_{max}$, we keep  $k_{max}$ learnable input features: $\mcinputfeature(\ltr) \  \forall \ltr \in \{1 \ldots k_{max} \}$. 

%\textbf{Input Features: } 

\textbf{Message Passing Update:}
%on $\relationgraph$ for generating `relationship-aware' embeddings:} 
At step $t$, update the hidden state, $\rghidden_t(\mvrvalnode{\ltr})$, of each of the value nodes in $\mvrgraph$, by the concatenation,$m_t(\mvrvalnode{\ltr})$,  of average messages, $m^{\mvrredge{}{}}_t(\mvrvalnode{\ltr})$, received across edges of type $\mvrredge{}{} \in R$: 
$\rghidden_{t+1}(\mvrvalnode{\ltr}) = \rgupdatefn(\rghidden_t(\mvrvalnode{\ltr}), m_t(\mvrvalnode{\ltr}), \mvrinputfeature(\perm_\query[\ltr]))$, 
where $\rgupdatefn$ is the hidden state update function. Like \cite{palm&al18}, it always takes the initial embedding, $\mvrinputfeature(\perm_\query[\ltr])$,  of the value node $\mvrvalnode{\ltr}$ as one of the inputs.
%where $\mcinputfeature(\perm_\query[\ltr]))$ is the initial node feature. 
Notice that the message,
$m^{\mvrredge{}{}}_t(\mvrvalnode{\ltr})$, is the average of the messages, $\msgfunction_{\mvrredge{}{}}(\rghidden_t(\mvrvalnode{\ltr}), \rghidden_t(\mvrvalnode{\ltr'})) \ \forall \ \mvrredge{\ltr}{\ltr'} \in \mvredges$, where $\msgfunction_{\mvrredge{}{}}$ is the message passing function for edge type $\mvrredge{}{} \in R$.
%The same function is used during the message passing in $\mvgraph$ for computing messages across edges of type $\mvrredge{}{}$.
The hidden states are updated for $\tilde{T}$ steps and the final embeddings, $\rghidden_{\tilde{T}}(\mvrvalnode{\ltr}) \ \forall v_\ltr \in \dspace$, are used as `relationship-aware' embeddings for initializing the input features (embeddings) of both variable nodes, $\mvnode{\jtr}$, and value nodes, $\mvvalnode{\ltr}$ in the graph $\mvgraph$.

\subsubsection{Recurrent Message Passing (CMPG)}
\textbf{Initialization:} Initialize the embedding of value nodes, $\mvvalnode{\ltr}$ in $\mvgraph$, using the  `relationship-aware' embeddings, $\rghidden_{\tilde{T}}(\mvrvalnode{\ltr})$, of $\mvrvalnode{\ltr}$ in $\mvrgraph$.
The variable nodes that are preassigned a value in $\query$, are initialized by the embedding of the corresponding value node, \ie, if $\query[\jtr] = \ltr$, then $\mvnode{\jtr}$ is initialized with the `relationship-aware' embedding, $\rghidden_{\tilde{T}}(\mvrvalnode{\ltr})$ , of $\mvrvalnode{\ltr}$.
On the other hand, the embedding of nodes corresponding to the unassigned variables are initialized by the average, $(1/k)\sum_{
v_\ltr \in \dspace} \rghidden_{\tilde{T}}(\mvrvalnode{\ltr})$, of all `relationship-aware' embeddings.
For a variable node $\mvnode{\jtr}$, we denote its initial embedding as:
$\inpfeature(\mvnode{\jtr})$.
Initialize the hidden state, $h_0(\mvvalnode{\ltr})$, for each value node $\mvvalnode{\ltr}$ in $\mvgraph$, with
a $0$ vector.
%$\rghidden_{T_R}(\ltr), \ \forall v_\ltr \in \dspace$.

\textbf{Message Passing in Update:}
At time step $t$, similar to \binarymodel, each node receives messages from its neighbors, that are aggregated based on the edge type.
For each node, the aggregated messages, $m_{t,\mvedgetype{}{}}(\mvnode{\jtr})$, for different edge types, $\mvedgetype{}{} \in (Q \cup A)$, are stacked to create, $m_t(\mvnode{\jtr})$, which updates the hidden state as:
\begin{equation}
    h_{t+1}(\mvnode{\jtr}) = 
    g\left(
    h_t(\mvnode{\jtr}), m_{t}(\mvnode{\jtr}),
    \inpfeature(\mvnode{\jtr})
    \right), \forall \mvnode{\jtr} \in \mvvertices
\end{equation}

\subsubsection{Loss Computation and Final Prediction}
At time step $t$, a scoring function, $s$, computes a score, $s(h_t(\mvnode{\jtr}), h_t(\mvvalnode{\ltr}))$,  for assigning a value $v_\ltr$ to a variable $\mvnode{\jtr}$ based on the hidden state of corresponding value and variable nodes.
For each variable node, a $Softmax$ converts these scores into probabilities over the values $v_\ltr \in \dspace$, \ie, $Pr(\mvnode{\jtr}.v = v_\ltr) = Softmax(s(h_t(\mvnode{\jtr}), h_t(\mvvalnode{\ltr}))), \  \forall v_\ltr \in \dspace_k$, 
where, $\mvnode{\jtr}.v \in \dspace$ denotes the value that node $\mvnode{\jtr}$ can take.
Total loss at step $t$ is nothing but the average of standard Cross Entropy over variable nodes:
$L_t= - \frac{1}{|\mvvertices|}\sum_{\mvnode{\jtr} \in \mvvertices} \log Pr(\mvnode{\jtr}.v= \target[\jtr])$. 

{\em Orthogonality Loss:} To ensure that the \multimodel\ learns different embeddings for each value in the domain, we add an auxiliary loss term, corresponding to the total pairwise dot product (similarity) of any two embeddings, before and after message passing in
$\mvrgraph$. 
We call it orthogonality loss. Its weight, $\alpha$, is a hyper-parameter.

\subsubsection{Relative Comparison}
%Drawbacks of \binarymodel}
In the \binarymodel, the constructed graph $\bingraph$ has $k|\vertices|$ nodes and at least $k|\edges| +  |\vertices|k(k-1)/2$ edges due to binarization of nodes. This increases the graph size by a factor of at least $k$. As a result, we may soon hit the memory limits of a GPU while training the \binarymodel\ with bigger problems. The model may also need significantly more inference time due to its bigger size. On the other hand, \multimodel\ , while being compact in terms of its representation, needs to learn additional embeddings, for a speculative test domain size. This poses additional requirement on the model both in terms of representation, and learning, possibly affecting the quality of generalization. While this is a simple analytical understanding of the possible merits of the two models, we would like to examine experimentally the impact of these issues on real datasets. 
%This is presented in the next section.



==> sections/s4_experiments_orig.tex <==
\section{Experiments}

\subsection{Data}

We introduce the task of domain-invariant puzzle solving in order to evaluate the two models proposed in Section 3. Specifically, we consider 3 sets of puzzles and contribute novel datasets for each set.

%1) Sudoku 2) Graph Coloring Problem and 3) Futoshiki. 

\subsubsection{Sudoku}
A general Sudoku puzzle consists of a $n \times n$ grid containing given clues in various places. The objective is to fill all empty squares so that the numbers $1$ to $n$ appear exactly once in each row, column and irregular shaped box. We discuss domain-invariance over grid-size $n$ by training on sudoku boards of grid-size $9$ and performing zero-shot evaluation on boards with bigger grid-sizes. 


\subsubsection{Graph Coloring Problem}
The GCP-based puzzle consists of a graph with $n$ nodes and $k$ colours. A partial assignment from nodes to colours is provided. The objective is to provide a complete assignment from nodes to colours so that no two adjacent vertex have the same colour. For the case of GCP, we focus on domain-invariance over number of colors, $k$, as well as graph size, $n$.  

\subsubsection{Futoshiki}
A general Futoshiki puzzle consists of a $n \times n$ grid containing given clues in various places. We are additionally provided with inequality constraints between various pairs of adjacent boxes. The objective is to fill all empty squares so that the numbers $1$ to $n$ appear exactly once in each row and column whilst honouring the inequality constraints. Similar to Sudoku, the point of discussion is domain-invariance over grid-size $n$. 

Various dataset statistics are provided in Table 1. 

% \subsection{Evaluation}

% We consider 2 intuitive evaluation metrics: 
% \begin{enumerate}
%     \item \textbf{Point-wise accuracy}: Average percentage match with intended target. 
%     \item \textbf{Puzzle accuracy}: Percentage of puzzles solved correctly which are valid for the given query. 
    
% \end{enumerate}


\subsection{Training}

All experiments described in the section have been repeated with three different seed values. 

\subsubsection{Binary Model}

Given a puzzle-instance's primal constraint graph, we can construct a binary model with directed edges for the puzzle as described in section 3.1.1. The primal constraint graph for a GCP-puzzle is the input graph with each undirected edge replaced by an anti-parallel pair of directed edges. For Sudoku, the graph remains the same across instances for a given board-size; each variable-node is connected to all other variables in the same row, column and box. For Futoshiki, the input graph is heterogeneous and contains 3 types of directed edges: (1) edges connecting each variable-node to all other variable-nodes in the same row and column, (2) forward-inequality edges connecting variable-node-pairs tied with inequality constraints in the forward direction and (3) backward-inequality edges analogous to (2). 

The node features $x_i$ are initialised depending on the node-state: whether it's masked, 0 or 1. The network is run for 32 time steps and message passing is performed as described in Section 3.1.3. At every time step, the output function calculates a score for each node based on its hidden state. For each variable-node in the input primal constraint graph, we can view the scores of the corresponding k-inserted nodes as output logits for k classes. We optimise Binary Cross Entropy on the logits averaged over all variable-nodes and message-passing steps, (similar to RRN) via Adam. 

Move this to section 3.1.3??

For the case of GCP, there are multiple solutions for a puzzle-query. <Describe the min-loss, add-to-targetset strategy>


% x(c, j) = 
% \begin{cases} 
%       f(-1) & $variable j is masked$ \\
%       f(1) & c = v \\
%       f(0) & $otherwise$
% \end{cases}

==> sections/s4_experiments_origv2.tex <==
\section{Experiments}
The main goal of our experiments is to evaluate the effectiveness of the two proposed methods, \binarymodel\ and \multiclassmodel, for achieving domain-size invariance.
%and assess the performance gap between them, if any.
We also wish to seek how well our methods can represent relationships, if any, between the classes.
To answer these questions, we train both our models for three different combinatorial puzzles, \textit{viz.}, Sudoku, Futoshiki, and Graph Coloring. We train them using queries from a fixed domain-size, and evaluate on queries from a larger domain.  
The experiments on Futoshiki helps to answer the second question, as the puzzle contains ordering relationship, $\relation$, between some pairs of cells. We use the information that $\relationfn(\ctr_a,\ctr_b) = 1 \ \text{iff} \  \ctr_a < \ctr_b, \forall \ctr_a, \ctr_b \in \{1 \ldots k\}$.
Next, we describe the three datasets, along with the other details of both the architectures.

\subsection{Task Description and Datasets}
\textbf{Futoshiki:}
This is a number puzzle similar to sudoku: we have to place numbers $\{1 \ldots k\}$ on a $k \times k$ grid, such that no two cells in a row or column contain the same number. 
In addition, there may be an ordering constraint between two cells, which needs to be honored in the final solution.
The input has some of the grid cells already filled with a number and the task is to complete the grid, respecting the additional ordering constraint where ever it exists.
\textbf{Training Data:} 
We train our model on $6 \times 6$ puzzles, with the number of missing cells varying uniformly between $30 - 70\%$. The number of pairs with inequality constraint varying uniformly between $x -y$.
\textbf{Test Data:} 
We test our models on puzzles with board size ranging between $6$ to $12$. The number of missing cells varies between $x-y\%$, and the number of constraint edges vary between $a-b\%$, depending on the board size. 
Exact distribution of number of missing cells and number of constraint edges for each board size is provided in the supplement.
\textbf{Data Generation:}
To generate the data, we first randomly generate a completely filled $k \times k$ board and then randomly mask $m\%$ of the cells. We search for possible completions using \ycom{DFS and backtracking?}. To ensure uniqueness of solution, we reject the query as soon as we find its $2$ possible valid completions, and select it only when the search terminates with just one solution.
Finally, we insert appropriate ordering constraints between $x$ randomly picked pairs of cells.
The entire process is repeated by varying $k$ and $m$ until sufficient number of queries for each board with appropriate masking are generated.

\textbf{Sudoku:} To train the models for solving sudoku, we randomly select $10,000$ queries from the $9 \times 9$ dataset introduced in \citet{palm&al18}. It has a uniform distribution of number of masked cells, varying between $17$ and $33$.
\textbf{Test Data:} We test our models on $k' \times k'$ puzzles, with $k \in \{10,12,15,16\}$. 
Data generation process is similar to Futoshiki, with the distribution of missing cells varying between $x-y\%$ depending on the board size. 

\textbf{Graph Coloring (GCP):}
In this task we are given a partially colored graph along with the number of colors $k$, and the objective is to color rest of the nodes using $k$ colors such that no two adjacent nodes have the same color. 
We train our model on randomly generated $4-$colorable graphs, and test on $k'-$colorable graphs, with $k' \in {4,5,6,7}$.
Training data has graph with number of nodes varying uniformly between $x-y\%$, and number of masked nodes vary uniformly between $a-b\%$, depending on the graph size. 
To generate the data, we follow the procedure similar to \cite{}. 

\subsection{Training and Network Details}
In both the models, nodes are initialized with learnable $96$ dimensional embeddings, depending on their initial feature value.
Note that for \binarymodel, there are only $3$ learnable embeddings, corresponding to the three input features, $0,1$ and $-1$. On the other hand, for the \multiclassmodel, there are $k_{max} = 12, 16$, or $7$ learnable embeddings for Futoshiki, Sudoku and GCP, respectively. Out of $k_{max}$,  $k = 6, 9$ or $4$ embeddings are selected randomly to initialize the value nodes in the relationship graph $\relationgraph$ for the different tasks.
Message passing on $\relationgraph$ in the \multiclassmodel\ runs for $T_R = 1$ step, resulting in embeddings used to initialize the nodes of $\mcgraph$.
The message passing functions, $\msgfunction_{\binedgetype{}{}}$ and $\msgfunction_{\edgetype{}{}}$, are $3$ layer MLPs, similar to those in RRN, with a difference that there is a separate function for each edge type $\binedgetype{}{} \in \{ \binedge{}{}, \binposnedge{}{}, \binredge{}{}, \bindiffedge{}{} \}$ for \binarymodel\ and $\edgetype{}{} \in \{\edge{}{}, \redge{}{}, \assignededge{}{}, \naedge{}{}, \diffedge{}{} \}$ for \multiclassmodel.
In both the models, a layer normalized LSTM cell with hidden dimension $96$ acts as state update functions, $g$, $\rgupdatefn$.
Finally, the message passing on both, $\bingraph$ in \binarymodel\ and $\mcgraph$ in \multiclassmodel, runs for $T = 32$ steps during training, and till convergence during inference, up-to maximum $T_{max} = 100$ steps.

\textbf{Ambiguity in GCP dataset:} Note that in the GCP dataset, an input query may have more than one solution, out of which only one is provided. It may happen that the network discovers a solution different from what is given, and computing loss of the discovered solution w.r.t. the given solution may unnecessarily penalize the model. To avoid this, we assume access to an oracle for indicating if the model's prediction is a valid coloring or not. If it is, then we instead compute loss w.r.t. to this discovered solution, instead of the given one.


==> todolist.tex <==
1. inference time and memory comparison b/w the two methods:
2. Futoshiki: analysis of the Generator GNN.

